Distributed Multigrid Neural Solvers on Megavoxel Domains

We consider the distributed training of large-scale neural networks that serve as PDE solvers producing full field outputs. We specifically consider neural solvers for the generalized 3D Poisson equation over megavoxel domains. A scalable framework is presented that integrates two distinct advances. First, we accelerate training a large model via a method analogous to the multigrid technique used in numerical linear algebra. Here, the network is trained using a hierarchy of increasing resolution inputs in sequence, analogous to the 'V', 'W', 'F', and 'Half-V' cycles used in multigrid approaches. In conjunction with the multi-grid approach, we implement a distributed deep learning framework which significantly reduces the time to solve. We show the scalability of this approach on both GPU (Azure VMs on Cloud) and CPU clusters (PSC Bridges2). This approach is deployed to train a generalized 3D Poisson solver that scales well to predict output full-field solutions up to the resolution of 512x512x512 for a high dimensional family of inputs.

==> preamble.tex <==
\usepackage{xcolor} 
\usepackage{array}
\usepackage{amsfonts}
\usepackage{graphicx}

\usepackage{epstopdf}
\usepackage{tikz,pgfplots}
\usetikzlibrary{arrows,shapes,trees}
\usepackage{amsopn}
\usepackage{listings}
\usepackage{adjustbox}
\usepackage{longtable}
\usepackage{multirow}
\usepackage{tabulary}
\usepackage{minted}
\usepackage{hyperref}
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\usetikzlibrary{arrows,shapes,plotmarks}
\pgfplotsset{compat=1.8}
\usepackage{soul}
\usepackage{rotating}
\usepackage{url}
\usepackage{enumitem}
\usepackage[labelfont=bf,textfont=it]{caption}
\usepackage{subcaption}
\usepackage{csvsimple}
\usepackage{makecell}
\usepackage{lipsum}
\usepackage{natbib}
\usepackage{nicefrac}
\usepackage{verbatim}

\newcommand{\mynote}[3]{
	\textcolor{#2}{\fbox{\bfseries\sffamily\scriptsize#1}}
		{\small$\blacktriangleright$\textsf{\emph{#3}}$\blacktriangleleft$}
}


\newcommand{\Frontera}{\href{https://frontera-portal.tacc.utexas.edu/}{Frontera}}


\acmConference[SC 2021]{ACM Conference}{2021}{St. Louis, MO}%

\newcommand{\bg}[1]{\mynote{Baskar}{magenta}{#1}}
\newcommand{\hs}[1]{\mynote{Hari}{olive}{#1}}
\newcommand{\ks}[1]{\mynote{Kumar}{blue}{#1}}
\newcommand{\bk}[1]{\mynote{Biswajit}{teal}{#1}}
\newcommand{\mi}[1]{\mynote{Masado}{lime}{#1}}
\newcommand{\mf}[1]{\mynote{Milinda}{brown}{#1}}

\newcommand{\stri}{sedectree} 
\newcommand{\stra}{sedecant}

\newcommand{\tsort}{\textsc{TreeSort}}
\newcommand{\tsearch}{\textsc{TreeSearch}}
\newcommand{\tcons}{\textsc{TreeConstruction}}
\newcommand{\dtcons}{\textsc{DistTreeConstruction}}
\newcommand{\taux}{\textsc{AuxiliaryOctants}}
\newcommand{\tbal}{\textsc{TreeBalancing}}
\newcommand{\tdbal}{\textsc{DistTreeBalancing}}
\newcommand{\tghost}{\textsc{ComputeGhostElements}}
\newcommand{\teToe}{\textsc{BuildE2E}}
\newcommand{\teTon}{\textsc{BuildE2N}}

\newcommand{\dendrokt}{\textsc{Dendro-KT}}
\newcommand{\dendrite}{\textsc{Dendrite}}
\newcommand{\Intercepted}{\textsc{Intercepted }}
\newcommand{\In}{\textsc{In }}
\newcommand{\Out}{\textsc{Out }}


\newcommand{\hilbertcurve}{\textsc{Hilbert}}
\newcommand{\mortoncurve}{\textsc{Morton}}


\newcommand{\tsortmodified}{\textsc{TreeSortModified}}
\newcommand{\dtsortmodified}{\textsc{DistTreeSortModified}}
\newcommand{\tbucket}{\textsc{SFC\_Bucketing}}
\newcommand{\maxDepth}{\textsc{maxdepth}}
%\newcommand{\tsort_cons}{\textsc{OctreeConstruction}}
\newcommand{\ssort}{\textsc{SampleSort}}
\newcommand{\dsort}{\textsc{DistTreeSort}}
\newcommand{\note}[1]{\noindent\emph{\textcolor{purple}{hs: #1}}}
%\algrenewcommand\algorithmicrequire{\textbf{Input:}}
%\algrenewcommand\algorithmicensure{\textbf{Output:}}
%\algrenewcommand\algorithmicforall{\textbf{parallel for}}

\newcommand{\Intel}{Intel\textsuperscript{\textregistered}\xspace}
\newcommand{\snb}{Xeon\texttrademark\xspace}
\newcommand{\xphi}{Xeon Phi\texttrademark\xspace}
\newcommand{\Summit}{\href{https://www.olcf.ornl.gov/summit/}{Summit}}
\newcommand{\Aurora}{\href{http://aurora.alcf.anl.gov/}{Aurora}}
\newcommand{\Stampede}{\href{https://www.tacc.utexas.edu/systems/stampede2}{Stampede2 }}
\newcommand{\Titan}{\href{https://www.olcf.ornl.gov/titan/}{Titan}}
\newcommand{\petsc}{\href{https://www.mcs.anl.gov/petsc/}{PETSc}}

\newcommand{\octdomain}{\mathcal{N}^3}
%%

\newcommand{\Tau}{\mathcal{T}}
\newcommand{\adv}{\mathbf{a}}

\newdimen\HilbertLastX
\newdimen\HilbertLastY
\newcounter{HilbertOrder}

\def\DrawToNext#1#2{%
  \advance \HilbertLastX by #1
  \advance \HilbertLastY by #2
  \pgfpathlineto{\pgfqpoint{\HilbertLastX}{\HilbertLastY}}
  % Alternative implementation using plot streams:
  % \pgfplotstreampoint{\pgfqpoint{\HilbertLastX}{\HilbertLastY}}
}

% \Hilbert[right_x,right_y,left_x,left_x,up_x,up_y,down_x,down_y]
\def\Hilbert[#1,#2,#3,#4,#5,#6,#7,#8] {
  \ifnum\value{HilbertOrder} > 0%
  \addtocounter{HilbertOrder}{-1}
  \Hilbert[#5,#6,#7,#8,#1,#2,#3,#4]
  \DrawToNext {#1} {#2}
  \Hilbert[#1,#2,#3,#4,#5,#6,#7,#8]
  \DrawToNext {#5} {#6}
  \Hilbert[#1,#2,#3,#4,#5,#6,#7,#8]
  \DrawToNext {#3} {#4}
  \Hilbert[#7,#8,#5,#6,#3,#4,#1,#2]
  \addtocounter{HilbertOrder}{1}
  \fi
}

% \hilbert((x,y),order)
\def\hilbert((#1,#2),#3){%
  \advance \HilbertLastX by #1
  \advance \HilbertLastY by #2
  \pgfpathmoveto{\pgfqpoint{\HilbertLastX}{\HilbertLastY}}
  % Alternative implementation using plot streams:
  % \pgfplothandlerlineto
  % \pgfplotstreamstart
  % \pgfplotstreampoint{\pgfqpoint{\HilbertLastX}{\HilbertLastY}}
  \setcounter{HilbertOrder}{#3}
  \Hilbert[1mm,0mm,-1mm,0mm,0mm,1mm,0mm,-1mm]
  \pgfusepath{stroke}%
}


\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

%strongly recommended
%\numberwithin{theorem}{section}

\definecolor{cpu3}{HTML}{F44336}
\definecolor{cpu4}{HTML}{2196F3}
\definecolor{cpu1}{HTML}{4CAF50}
\definecolor{cpu2}{HTML}{FFC107}
\definecolor{gpu3}{HTML}{EF9A9A}
\definecolor{gpu4}{HTML}{90CAF9}
\definecolor{gpu1}{HTML}{A5D6A7}
\definecolor{gpu2}{HTML}{FFE082}

\definecolor{cpu5}{HTML}{9932CC}

\definecolor{sq_b1}{RGB}{37,52,148}
\definecolor{sq_b2}{RGB}{44,127,184}
\definecolor{sq_b3}{RGB}{65,182,196}
\definecolor{sq_b4}{RGB}{127,205,187}
\definecolor{sq_b5}{RGB}{199,233,180}
\definecolor{sq_b6}{RGB}{255,255,204}

\definecolor{sq_r1}{RGB}{189,0,38}
\definecolor{sq_r2}{RGB}{240,59,32}
\definecolor{sq_r3}{RGB}{253,141,60}
\definecolor{sq_r4}{RGB}{254,178,76}
\definecolor{sq_r5}{RGB}{254,217,118}
\definecolor{sq_r6}{RGB}{255,255,178}

\definecolor{sq_g1}{RGB}{0,104,55}
\definecolor{sq_g2}{RGB}{49,163,84}
\definecolor{sq_g3}{RGB}{120,198,121}
\definecolor{sq_g4}{RGB}{173,221,142}
\definecolor{sq_g5}{RGB}{217,240,163}
\definecolor{sq_g6}{RGB}{255,255,204}


\definecolor{div_c1}{RGB}{230,171,2}
\definecolor{div_c2}{RGB}{102,166,30}
\definecolor{div_c3}{RGB}{231,41,138}
\definecolor{div_c4}{RGB}{117,112,179}
\definecolor{div_c5}{RGB}{217,95,2}
\definecolor{div_c6}{RGB}{27,158,119}
\definecolor{div_c7}{RGB}{215,48,39}

\definecolor{div_d1}{RGB}{215,25,28}
\definecolor{div_d2}{RGB}{253,174,97}
\definecolor{div_d3}{RGB}{255,255,191}
\definecolor{div_d4}{RGB}{171,217,233}
\definecolor{div_d5}{RGB}{44,123,182}




\definecolor{lineclr}{RGB}{0,0,0}
\definecolor{utorange}{RGB}{0,0,255}
\definecolor{utsecblue}{RGB}{255,255,0}
\definecolor{utsecgreen}{RGB}{255,0,0}
\definecolor{red!15}{RGB}{0,255,255}
\definecolor{fillclr5}{RGB}{0,255,0}
\definecolor{fillclr6}{RGB}{255,0,255}
\definecolor{fillclr7}{RGB}{255,255,255}
\definecolor{fillclr8}{RGB}{0,0,0}

\newcommand{\tikzcircle}[2][red,fill=red]{\tikz[baseline=-0.5ex]\draw[#1,radius=#2] (0,0) circle ;}%



\def\drawcubeI(#1,#2,#3,#4,#5){ % x,y,z,sz,line color
\coordinate (O) at (#1,#2,#3);
\coordinate (A) at (#1,#2+#4,#3);
\coordinate (B) at (#1,#2+#4,#3+#4);
\coordinate (C) at (#1,#2,#3+#4);
\coordinate (D) at (#1+#4,#2,#3);
\coordinate (E) at (#1+#4,#2+#4,#3);
\coordinate (F) at (#1+#4,#2+#4,#3+#4);
\coordinate (G) at (#1+#4,#2,#3+#4);
\draw[#5] (O) -- (C) -- (G) -- (D) -- cycle;% Bottom Face
\draw[#5] (O) -- (A) -- (E) -- (D) -- cycle;% Back Face
\draw[#5] (O) -- (A) -- (B) -- (C) -- cycle;% Left Face
\draw[#5] (D) -- (E) -- (F) -- (G) -- cycle;% Right Face
\draw[#5] (C) -- (B) -- (F) -- (G) -- cycle;% Front Face
\draw[#5] (A) -- (B) -- (F) -- (E) -- cycle;% Top Face
}


\def\drawcubeII(#1,#2,#3,#4,#5,#6,#7){ % x,y,z,sz,line color,fill color,opacity
\coordinate (O) at (#1,#2,#3);
\coordinate (A) at (#1,#2+#4,#3);
\coordinate (B) at (#1,#2+#4,#3+#4);
\coordinate (C) at (#1,#2,#3+#4);
\coordinate (D) at (#1+#4,#2,#3);
\coordinate (E) at (#1+#4,#2+#4,#3);
\coordinate (F) at (#1+#4,#2+#4,#3+#4);
\coordinate (G) at (#1+#4,#2,#3+#4);
\draw[#5,fill=#6,opacity=#7] (O) -- (C) -- (G) -- (D) -- cycle;% Bottom Face
\draw[#5,fill=#6,opacity=#7] (O) -- (A) -- (E) -- (D) -- cycle;% Back Face
\draw[#5,fill=#6,opacity=#7] (O) -- (A) -- (B) -- (C) -- cycle;% Left Face
\draw[#5,fill=#6,opacity=#7] (D) -- (E) -- (F) -- (G) -- cycle;% Right Face
\draw[#5,fill=#6,opacity=#7] (C) -- (B) -- (F) -- (G) -- cycle;% Front Face
\draw[#5,fill=#6,opacity=#7] (A) -- (B) -- (F) -- (E) -- cycle;% Top Face
}




\def\drawNodes(#1,#2,#3,#4,#5,#6,#7){ % x_min,x_max,y_min,y_max,z_min,z_max,min+stepSz
\foreach \x in {#1,#7,...,#2}{
	\foreach \y in {#3,#7,...,#4}{
		\foreach \z in {#5,#7,...,#6}{
				\draw[fill=red!60] (\x,\y,\z) circle (0.15);
				}
			}
	}				
		
}


\makeatletter
\newcommand\resetstackedplots{
\makeatletter
\pgfplots@stacked@isfirstplottrue
\makeatother
\addplot [forget plot,draw=none] coordinates{(48,0) (96,0) (192,0) (384,0) (768,0) (1536,0) (3072,0) (6144,0)};
}
\makeatother

\makeatletter
\newcommand\resetstackedplotsOne{
\makeatletter
\pgfplots@stacked@isfirstplottrue
\makeatother
\addplot [forget plot,draw=none] coordinates{(384,0) (768,0) (1536,0) (3072,0) (6144,0)};
}
\makeatother

\makeatletter
\newcommand\resetstackedplotsTwo{
\makeatletter
\pgfplots@stacked@isfirstplottrue
\makeatother
\addplot [forget plot,draw=none] coordinates{(16,0) (32,0) (64,0) (128,0) (256,0) (512,0) (1024,0) (2048,0) (4096,0) (8192,0) (16384,0) (32768,0)};
}
\makeatother


\makeatletter
\newcommand\resetstackedplotsThree{
\makeatletter
\pgfplots@stacked@isfirstplottrue
\makeatother
\addplot [forget plot,draw=none] coordinates{(2,0) (4,0) (8,0) (16,0) (32,0) (64,0)};
}
\makeatother


\makeatletter
\newcommand\resetstackedplotsFour{
\makeatletter
\pgfplots@stacked@isfirstplottrue
\makeatother
\addplot [forget plot,draw=none] coordinates{(4,0) (8,0) (16,0) (32,0) (64,0)};
}
\makeatother

\makeatletter
\newcommand\resetstackedplotsFive{
\makeatletter
\pgfplots@stacked@isfirstplottrue
\makeatother
\addplot [forget plot,draw=none] coordinates{(1,0) (2,0) (4,0) (8,0) (16,0) (32,0) (64,0) (128,0)};
}
\makeatother

\makeatletter
\newcommand\resetstackedplotsSix{
\makeatletter
\pgfplots@stacked@isfirstplottrue
\makeatother
\addplot [forget plot,draw=none] coordinates{(2,0) (4,0) (8,0) (16,0) (32,0) (64,0) (128,0)};
}
\makeatother

\newcommand{\ipoint}[1]{{\color{blue}\textbf{#1}}}

\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}


==> previous_work/Data/MatrixAssemblyData.tex <==
\begin{figure}[h]
\centering
\begin{tikzpicture}[
  every axis/.style={
    ybar stacked,
    ymin=0,ymax=17,
    ylabel = Time (in s),
    x tick label style={
       % add some negative yshift to move ticklabels down
       yshift=-4mm,
       rotate=45,
       anchor=east},
%   x axis line style = { opacity = 0 }, 
%   y axis line style = { opacity = 0 },
  tickwidth = 0pt,
  legend style={
    legend columns=2,
        yshift=0mm,
        xshift = -40 mm,
        anchor=north,
        draw=none
    },
%   width=15cm,
%   height=8cm,
  % symbolic coords have numerical distance of 1
  % so with the following line you get a tick at every symbolic coord
  xtick distance=1,
  symbolic x coords={
      Skx Stampede,
      SkyLake Frontera,
      KNL stampede,
    },
  bar width=6pt
  },
]

\pgfplotsset{
  % define a new style used for the plot used to add labels
  % 2 args means it takes two mandatory arguments, so must be used as
  % labelplot={first arg}{second arg}
  labelplot/.style 2 args={
     % forget plot means it doesn't affect cycle lists or legends
     forget plot,
     % #1 is first argument, the text used in the nodes near coords
     nodes near coords=#1,
     % #2 is second argument, a length that should be the same as the bar shift for the axis
     every node near coord/.style={below,font=\tiny,xshift=#2}
  }
}
% Without Tensor
\begin{axis}[bar shift=-12pt, xticklabels={}]
\addplot [labelplot={GP}{-12pt}] coordinates
{(Skx Stampede,0) (SkyLake Frontera,0) (KNL stampede,0)};
\addplot coordinates
{(Skx Stampede,1.0617e+00) (SkyLake Frontera,8.0538e-01) (KNL stampede,5.4996e+00)};
\addplot coordinates
{(Skx Stampede,3.1981) (SkyLake Frontera,2.33232) (KNL stampede,9.5344)};
\end{axis}

\begin{axis}
\addplot [labelplot={MM}{0pt}] coordinates
{(Skx Stampede,0) (SkyLake Frontera,0) (KNL stampede,0)};
\addplot coordinates
{(Skx Stampede,7.7540e-01) (SkyLake Frontera,5.6241e-01) (KNL stampede,3.7750e+00)};
\addplot coordinates
{(Skx Stampede,3.1447) (SkyLake Frontera,2.56089) (KNL stampede,9.616 )};
\legend{Assembly time, Total solve time}
\end{axis}
\end{tikzpicture}
 \caption{Comparison of time on different cluster for matrix assembly and complete solve time for linear basis function.}
 \label{fig:MatAssemblyLinear}
\end{figure}

\begin{figure}
\begin{tikzpicture}[
  every axis/.style={
    ybar stacked,
    ymin=0,ymax=700,
    ylabel = Time (in s),
    x tick label style={
       % add some negative yshift to move ticklabels down
       yshift=-4mm,
       rotate=45,
       anchor=east},
        legend style={
    legend columns=2,
        yshift=0mm,
        xshift = -40 mm,
        anchor=north,
        draw=none
    },
%   x axis line style = { opacity = 0 }, 
%   y axis line style = { opacity = 0 },
  tickwidth = 0pt,
%   width=15cm,
%   height=8cm,
  % symbolic coords have numerical distance of 1
  % so with the following line you get a tick at every symbolic coord
  xtick distance=1,
  symbolic x coords={
      Skx Stampede,
      SkyLake Frontera,
      KNL stampede,
    },
  bar width=6pt
  },
]

\pgfplotsset{
  % define a new style used for the plot used to add labels
  % 2 args means it takes two mandatory arguments, so must be used as
  % labelplot={first arg}{second arg}
  labelplot/.style 2 args={
     % forget plot means it doesn't affect cycle lists or legends
     forget plot,
     % #1 is first argument, the text used in the nodes near coords
     nodes near coords=#1,
     % #2 is second argument, a length that should be the same as the bar shift for the axis
     every node near coord/.style={below,font=\tiny,xshift=#2}
  }
}
\begin{axis}[bar shift=-12pt, xticklabels={}]
\addplot [labelplot={GP}{-12pt}] coordinates
{(Skx Stampede,0) (SkyLake Frontera,0) (KNL stampede,0)};
\addplot coordinates
{(Skx Stampede,7.1132e+01) (SkyLake Frontera,5.9356e+01) (KNL stampede,3.8559e+02)};
\addplot coordinates
{(Skx Stampede,163.078) (SkyLake Frontera,153.414) (KNL stampede,278.46)};
\end{axis}

\begin{axis}
\addplot [labelplot={MM}{0pt}] coordinates
{(Skx Stampede,0) (SkyLake Frontera,0) (KNL stampede,0)};
\addplot coordinates
{(Skx Stampede,1.0245e+01) (SkyLake Frontera,8.4647e+00) (KNL stampede,4.0409e+01)};
\addplot coordinates
{(Skx Stampede,164.785) (SkyLake Frontera,155.9953) (KNL stampede,305.741 )};
\legend{Assembly time, Total solve time}
\end{axis}
\end{tikzpicture}
 \caption{Comparison of time on different cluster for matrix assembly and complete solve time for quadratic basis function. GP indicates the assembly over looping over the individual Gauss points and MM indicates the assembly by imposing FEM operator as matrix - matrix multiplication.}
 \label{fig:MatAssemblyQuad}
\end{figure}



==> previous_work/Result.tex <==
One of the key outcome of our experiments was to demonstrate a practical approach to train DiffNets on domain sizes $> 512 \times 512$ that are too big for GPUs. We tested our framework on both TACC \textbf{Stampede2} HPC clusters with bare-metal access, as well as \textbf{Microsoft Azure} and \textbf{Amazon Web Services} (AWS) HPC clusters built using on-demand virtual machines. We target these computational resources as representative of what is easily accessible for the general data science practitioner unlike DGX-2 that requires significant investment. We report results obtained from Microsoft Azure and Stampede2. On Table \ref{tab:azure_vs_stampede_specs}, we provide all relevant specifications for Azure and Stampede2 used in our experiments. We present wall-clock time comparisons between Azure and Stampede2 in section \ref{subsec:conventional_cloud} to determine the cluster to use for our large domain runs. In section \ref{subsec:strong_scaling}, we conduct strong scaling experiments for $128 \times 128$ and $256 \times 256$ domain sizes for 1 to 128 nodes (48 to 6144 cores) on Stampede2 to demonstrate scalability of our software. Finally, in section \ref{subsec:high_resolution_diffnet}, we present results for training a DiffNet model for \textbf{$512 \times 512$} and \textbf{$1024 \times 1024$} domain sizes for Burgers' inviscid equation (Eq.~\ref{eq:Inviscid_Burgers}) for parameter distributions characterizing the initial conditions (Eq.~\ref{eq:initial-condition}), which are currently not possible to train on GPUs.

\begin{table}[!ht]
  \begin{center}
    \begin{tabular}{|c|c|c|}
    \hline
     {\bf Specification} & {\bf Microsoft Azure}  & {\bf Stampede2} \\
     \hline
     Type & Virtual Machine & Bare-Metal \\
     \hline
     CPU & Intel Xeon Platinum 8168 & Intel Xeon Platinum 8160 \\
     \hline
     CPU cores & 44 & 48 \\
     \hline
     Memory (GB)& 352& 192\\
     \hline
     Interconnect & EDR Infiniband & Intel Omni-Path \\
     \hline
     Bandwidth & 100 Gb/sec & 100 Gb/sec \\
     \hline
     Topology & Fat tree & Fat tree \\
     \hline
\end{tabular}
\caption{Functional specifications of Microsoft Azure and Stampede2 infrastructure used in our experiments. \label{tab:azure_vs_stampede_specs}}
\end{center}
\end{table}
\subsection{Conventional HPC vs. Cloud Based HPC} 
\label{subsec:conventional_cloud}
In this section, we compare wall-clock times between Microsoft Azure and Stampede2 in order to determine the optimal HPC cluster configuration to train \emph{DiffNet} with very large ($1024\times 1024$) resolutions. On Table \ref{tab:azure_vs_stampede}, we show per-epoch wall-clock times (in seconds) to train DiffNet with $64\times 64$ resolution using 1, 2 and 4 nodes. The total number of samples used for this experiment was $N_s = 4096$ and the global batch size was $b_s = 1024$; the number of processes per node was fixed at 4, with each process spawning 8 local threads. Single node performance on bare-metal Stampede2 is $\sim 2 \times$ faster than on Azure VM. On the same table, we also compare per-epoch wall-clock times (in seconds) for different resolutions on 4 compute nodes (with 4 processes per node, 8 threads per process). Even though the infrastructure specifications of Azure and Stampede2 are almost identical, slowness on Azure can be attributed to the overheads associated with virtual machines.

\begin{table}[!ht]
  \begin{center}
    \begin{tabular}{|c|c|c|c|}
    \hline
     {\bf Domain Size} & {\bf Nodes} & {\bf Azure} & {\bf Stampede2}  \\
     \hline
     64x64 & 1 &113.1&67.2 \\
     \hline
     64x64 & 2 &54.9&34.9 \\
     \hline
     64x64 & 4 & 28.6& 19.4\\
     \hline
     128x128 & 4& 126.2 &68.5 \\
     \hline
     256x256 & 4 & 597.6& 279.8\\
     \hline
\end{tabular}
\caption{Comparison of per-epoch wall-clock times (in seconds) between Azure and Stampede2 for varying resolutions and different number of nodes (see Table \ref{tab:azure_vs_stampede_specs} for cluster specs). For both clusters, 4 processes were used per node (spawning 8 threads each). \label{tab:azure_vs_stampede}}
\end{center}
\end{table}

\subsection{Scaling Experiments} 
\label{subsec:strong_scaling}
In Figure \ref{fig:sc_strong_scaling}, we report strong scaling results to train {\it DiffNet} for $128\times 128$ and $256\times 256$ resolutions, using from 4 to 128 nodes on Stampede2. In this experiment, we used 8 MPI processes per node and each process spawned 12 threads, to a total of 96 threads per node. This matches the full capacity of the Stampede2 Skylake nodes, which have 48 physical hyperthread-enabled CPU cores, resulting in 96 hardware threads per node. On Table \ref{tab:wall_clock_times}, we show comparisons of wall clock times per epoch between GPU and Stampede2 using SciDDL. 
\begin{figure}[!ht]
  \centering
  \includegraphics[width=0.45\textwidth]{Figures/sc_strong_scaling.jpg}
  \caption{Strong scaling results for training {\it DiffNet} on Stampede2: per-epoch times (in seconds) versus number of nodes for $128\times 128$ and $256\times 256$ resolutions, using 8 processes per node and 12 threads per process.\label{fig:sc_strong_scaling}}
\end{figure}


\begin{table}[!ht]
  \begin{center}
    \begin{tabular}{|c|c|c|c|}
    \hline
     {\bf Output resolution} &   {\bf GPU (seconds)} & {\bf SciDDL (seconds)} \\
     \hline
     128$\times$128 & 105 & 4.6\\
     \hline
     256$\times$256	& 340 & 12.7\\
     \hline
     512$\times$512	& 1401 & 25.3 \\
     \hline
     1024$\times$1024 & N/A & 89.5 \\
     \hline
\end{tabular}
\caption{Comparison of per-epoch wall-clock time  between Titan RTX GPU and SciDDL on 128 Stampede2 nodes to train Diffnet (of different resolutions) with 4096 samples. Training on large CPU clusters using SciDDL is $20-60\times$ faster than training on the Titan RTX GPU.\label{tab:wall_clock_times}}
\end{center}
\end{table}

% \begin{table}[!ht]
%   \begin{center}
%     \begin{tabular}{|c|c|c|c|}
%     \hline
%      {\bf Domain Size} &   {\bf FEM (seconds)} & {\bf SciDDL (seconds)} \\
%      \hline
%     %  128$\times$128 & 105 & 4.6\\
%     %  \hline
%     %  256$\times$256	& 340 & 12.7\\
%     %  \hline
%      512$\times$512	& 23.2 & 3.6 \\
%      \hline
%      1024$\times$1024 & 395.6 & 9.8 \\
%      \hline
% \end{tabular}
% \caption{Comparison of solve time for the finite element solution  and the inference time for the SciDDL solution \label{tab:comparison_FEM_ML}}
% \end{center}
% \end{table}

As discussed in section \ref{subsec:complexities}, our computation time complexity scales with $p$ and communication complexity is independent of $p$. In Figure \ref{fig:comp_vs_comm_wc_times_256x256}, we show the computation and communication wall-clock times for different $p$. We observed that our communication times reduce with $p$ while we expected them to be constant. We do not have an explanation for this behavior at the time of this writing. However, we are actively investigating if this can be attributed to internal node-aware improvements \cite{node_aware_allreduce} to \emph{MPI\_Allreduce}.

\begin{figure}[!ht]
  \centering
  \includegraphics[width=0.45\textwidth]{Figures/comp_vs_comm_wc_times_256x256.png}
  \caption{Computation and communication wall clock times for different $p$ corresponding to strong scaling results for domain size $256 \times 256$ in Figure \ref{fig:sc_strong_scaling}. Computation time scales linearly with $p$ while communication time decreases with $p$, although we expected it to be independent of $p$. We are actively investigating this behavior and do not have an explanation for this at the time of this writing. \label{fig:comp_vs_comm_wc_times_256x256}}
\end{figure}

% \begin{figure}[!ht]
%   \centering
%   \includegraphics[width=0.45\textwidth]{Figures/loss_vs_epoch_128x128.png}
%   \caption{Loss vs. Epoch for 128x128 placeholder to demonstrate loss preservation independent of $p$ \label{fig:loss_vs_epoch_128x128}}
% \end{figure}
As discussed in section \ref{subsec:data_parallel_ddl}, the training samples are split in such a way as to guarantee loss decay integrity, i.e., the same exact problem is solved independently of the number of MPI processes. In Figure \ref{fig:loss_vs_epoch_256x256}, we show the loss vs. epoch for different values of $p$. The small deviation in loss values for different $p$ is due to rounding errors in \emph{MPI\_Allreduce} operations for computing gradient averages.

\begin{figure}[!ht]
  \centering
  \includegraphics[width=0.45\textwidth]{Figures/loss_vs_epoch_256x256.png}
  \caption{Comparison of loss decay vs. epoch for a subset of $p$ used in strong scaling experiments in Figure \ref{fig:sc_strong_scaling}. Loss decay is preserved (independent of $p$). \label{fig:loss_vs_epoch_256x256}}
\end{figure}

% \begin{figure}[!ht]
%   \centering
%   \includegraphics[width=0.45\textwidth]{Figures/loss_vs_epoch_error_256x256.png}
%   \caption{Maximum relative error in loss per epoch across for different $p$. These errors are bounded and are attributed to rounding errors in \emph{MPI\_Allreduce}. \label{fig:loss_vs_epoch_error_256x256}}
% \end{figure}

\subsection{High Resolution DiffNet} 
\label{subsec:high_resolution_diffnet}
In this sub-section, we illustrate the ability of the framework to train {\it DiffNet} models with very high resolution outputs (sizes $\ge 512\times 512$). This typically requires $\ge 2000$ epochs until convergence (for different ranges of the initial condition frequency $c$).

{\bf Example 1:} In the first example, we train a DiffNet to produce outputs of resolution $1024 \times 1024$. We emphasize that generative models of this size have hitherto fore not been trained (to the best of our knowledge). We train the DiffNet to be predictive in a range of the parameter $c\in [3,6]$. We remind the reader that $c$ represents a one-parameter family of initial conditions to the inviscid Burgers equation. The training sample set consists of 256 points from $c\in [3,6]$. We set the mini-batch size to 64. This model was trained on 8 nodes of Stampede2 (with 8 processes per node), taking 2200 epochs till convergence (see Fig.~\ref{fig:loss_1024}). The runtime for this training was 32 hours. 
\begin{figure}[h]
  \centering
  \includegraphics[width=0.45\textwidth]{Figures/loss_1024.jpg}
  \caption{Loss vs. epoch for training DiffNet with domain size $1024\times 1024$ on Stampede2 using 256 sample points and batch size 64.\label{fig:loss_1024}}
\end{figure}

\begin{figure*}[ht]
\centering
\captionsetup{justification=centering}
    \begin{subfigure}{0.49\textwidth}
      \centering
      \subcaption*{SciDDL solution}
      \includegraphics[trim=80 50 80 80,clip,width=1.0\linewidth]{Figures/comparison_images/ml-m1024-c03.png}
    %   \caption{}
    %   \label{fig:ST-Diff3D}
    \end{subfigure}
    %\\
    \begin{subfigure}{0.49\textwidth}
      \centering
      \subcaption*{Finite element solution}
      \includegraphics[trim=80 50 80 80,clip,width=1.0\linewidth]{Figures/comparison_images/fe-m1024-c3.png}
    %   \caption{}
    %   \label{fig:ST-Adv3D}
    \end{subfigure}
    \caption{Inviscid Burgers' equation  solved on $1024\times1024$ pixels (left) or elements (right)}
    \label{fig:comparison-panel_1024}
\end{figure*}

After training, we performed inference using the DiffNet for a set of initial conditions from the one-parameter family. Results for $c = 3$ are shown in Fig.~\ref{fig:comparison-panel_1024}, where we compare the DiffNet inference result with the solution from an optimized FEM solver (based on the Petsc library) of the inviscid Burgers equation. While the general trend of the solution (as the wave evolves -- from left to right in the figures -- and forms shocks) is captured well, there is still room for improvement as the more diffused nature of the ML solution indicates. We hypothesize that using higher order Sobel filters (i.e. computing the gradients using higher order stencils) could help in eliminating the diffusive features of the ML solution. We continue to explore these aspects and hope to include them in the revised manuscript. 

% Results for $1024\times 1024$ resolution: 256 training examples, mini-batch size 64, $c\in [3,6]$; 64 processes, 8 nodes (Stampede2); ran to 2200 epochs (32hrs runtime).

% \begin{figure}[!ht]
%   \centering
%   \includegraphics[width=0.45\textwidth]{Figures/result_1024_c_3.jpg}
%   \caption{Inviscid Burgers' solution for $1024\times 1024$ and $c=3$ \label{fig:result_1024_c_3}}
% \end{figure}

% \begin{figure}[!ht]
%   \centering
%   \includegraphics[width=0.45\textwidth]{Figures/result_1024_c_3_3D.jpg}
%   \caption{Inviscid Burgers' solution for $1024\times 1024$ and $c=3$ \label{fig:result_1024_c_3_3D}}
% \end{figure}


{\bf Example 2:} In the second example, we explore if the DiffNet can be trained to predict solutions for a much larger distribution of the initial conditions. We train a DiffNet to predict solutions at $512\times 512$ resolution, but for initial conditions from $c\in [3,16]$. At higher values of c (which represent initial conditions exhibiting higher frequencies), we expect the formation of multiple shocks. The traditional numerical solutions for these initial conditions have to be carefully performed. We set the mini-batch size to 64. This model was trained on 8 nodes (64 processors) on Stampede2, taking 4000 epochs till convergence (see Fig.~\ref{fig:loss_512}). The runtime for training this model was 15 hours. Notice that the loss in this case is significantly larger than the previous example. This is due to two reasons: the reduced resolution ($1024 \rightarrow 512$) and, more importantly, the larger $c$ space.  
\begin{figure}[h]
  \centering
  \includegraphics[width=0.45\textwidth]{Figures/loss_512.jpg}
  \caption{Loss vs. epoch for training DiffNet with domain size $512\times 512$ on Stampede2 using 256 sample points and batch size 64.\label{fig:loss_512}}
\end{figure}

After training, we again performed inference using the DiffNet for a set of initial conditions from the one-parameter family. Results for $c = 3, 5, 10, 13$ are shown in Fig.~\ref{fig:comparison-panel}, where we compare the DiffNet inference result with the solution from an optimized FEM solver (based on the Petsc library) of the inviscid Burgers equation. As before, the general trend of the solution (as the wave evolves -- from left to right in the figures -- and forms shocks) is captured well, but there is still room for improvement. What we find very promising is that the DiffNet is able act as a general PDE solver for a wide range of initial conditions. This strongly suggests that, with the proper training infrastructure, it is possible to develop truly general PDE solvers that produce accurate solutions for general classes of PDE's.

{\bf Comparison of run-times between DiffNet and FEM based solutions}: While the training times for ML models is admittedly long, once trained, the inference step is often very fast. This allows one to amortize the cost of training across multiple users and instances. The availability of a general 'NeuralPDE' makes this a viable possibility. We quantify this argument by comparing the time it takes for a trained DiffNet to make a prediction (i.e. inference) with the time it takes for a well optimized FEM solver to perform the same prediction. 

\begin{figure*}[!ht]
\centering
\captionsetup{justification=centering}
    \begin{subfigure}{0.4\textwidth}
      \centering
      \subcaption*{SciDDL solution}
      \includegraphics[trim=30 0 0 30,clip,width=1.0\linewidth]{Figures/comparison_images/small/ml-m512-c03-small.png}
    %   \caption{}
    %   \label{fig:ST-Diff3D}
    \end{subfigure}
    %\\
    \begin{subfigure}{0.4\textwidth}
      \centering
      \subcaption*{Finite element solution}
      \includegraphics[trim=30 0 0 30,clip,width=1.0\linewidth]{Figures/comparison_images/small/fe-m512-c03-small.png}
    %   \caption{}
    %   \label{fig:ST-Adv3D}
    \end{subfigure}
    \\
    \begin{subfigure}{.4\textwidth}
      \centering
      \includegraphics[trim=30 0 0 30,clip,width=1.0\linewidth]{Figures/comparison_images/small/ml-m512-c05-small.png}
    %   \caption{}
    %   \label{fig:ST-AC3D}
    \end{subfigure}
    %\\
    \begin{subfigure}{.4\textwidth}
      \centering
      \includegraphics[trim=30 0 0 30,clip,width=1.0\linewidth]{Figures/comparison_images/small/fe-m512-c05-small.png}
    %  \caption{}
    %   \label{fig:ST-Diff-slice}
    \end{subfigure}
    \\
    \begin{subfigure}{.4\textwidth}
      \centering
      \includegraphics[trim=30 0 0 30,clip,width=1.0\linewidth]{Figures/comparison_images/small/ml-m512-c10-small.png}
    %   \caption{}
    %   \label{fig:ST-Adv-slice}
    \end{subfigure}
    %\\
    \begin{subfigure}{.4\textwidth}
      \centering
      \includegraphics[trim=30 0 0 30,clip,width=1.0\linewidth]{Figures/comparison_images/small/fe-m512-c10-small.png}
    %   \caption{}
    %   \label{fig:ST-AC-slice}
    \end{subfigure}
    \\
    \begin{subfigure}{.4\textwidth}
      \centering
      \includegraphics[trim=30 0 0 30,clip,width=1.0\linewidth]{Figures/comparison_images/small/ml-m512-c13-small.png}
    %   \caption{}
    %   \label{fig:ST-Adv-slice}
    \end{subfigure}
    %\\
    \begin{subfigure}{.4\textwidth}
      \centering
      \includegraphics[trim=30 0 0 30,clip,width=1.0\linewidth]{Figures/comparison_images/small/fe-m512-c13-small.png}
    %   \caption{}
    %   \label{fig:ST-AC-slice}
    \end{subfigure}
    \caption{Contour plots of the solution to the inviscid Burgers' equation: solutions from DiffNet (left) vs solutions from a finite element solver (right). The initial condition is characterized by the wave number $c$ (defined in \ref{eq:initial-condition}). The first row presents solution for $c = 3$ and subsequently for $c$ = 5, 10 and 13 in the latter rows respectively. On the left, the image size is $512\times512$ pixels, whereas on the right, the discretization is a mesh of $512\times512$ bilinear quadrilateral elements.}
    \label{fig:comparison-panel}
\end{figure*}
\clearpage

This comparison is reported in Table~\ref{tab:comparison_FEM_ML}, which shows a 40x improvement in prediction time. We emphasize that the inference step is not optimized, suggesting that the 40x improvement we show is a lower bound. 

\begin{table}[!ht]
  \begin{center}
    \begin{tabular}{|c|c|c|c|}
    \hline
     {\bf Domain Size} &   {\bf FEM (seconds)} & {\bf SciDDL (seconds)} \\
     \hline
    %  128$\times$128 & 105 & 4.6\\
    %  \hline
    %  256$\times$256	& 340 & 12.7\\
    %  \hline
     512$\times$512	& 23.2 & 3.6 \\
     \hline
     1024$\times$1024 & 395.6 & 9.8 \\
     \hline
\end{tabular}
\caption{Comparison of solve time for the finite element solution  and the inference time for the SciDDL solution \label{tab:comparison_FEM_ML}}
\end{center}
\end{table}

\section{Conclusions}
In this work, we report on a data distributed computing approach for training large neural network architectures, especially in the context of data-free generative models that serve as PDE solvers. We  highlighted  some of the key challenges and improvements over conventional GPU based training strategies, as well as other data-parallel approaches. We demonstrated excellent scaling  results  for  our  framework  on current  supercomputers. We illustrated the ability of this framework to enable practitioners to train very large models, thus enabling practical applications of such 'neuralPDE' solvers. We  believe  that availability of tools like the one presented here will help democratize the ability of a data scientist to produce (near) real time predictions of complex systems characterized by PDEs. Our future goals include extension of the framework to include higher order solvers (i.e. beyond Stochastic Gradient Descent) to methods like L-BFGS which need very large memory (which CPU clusters provide), as well as incorporating model parallelism for increased scaleup.



==> previous_work/Result_revised.tex <==
One of the key outcome of our experiments was to demonstrate a practical approach to train DiffNets on domain sizes $> 512 \times 512$ that are too big for GPUs. We tested our framework on both TACC \textbf{Stampede2} HPC clusters with bare-metal access, as well as \textbf{Microsoft Azure} and \textbf{Amazon Web Services} (AWS) HPC clusters built using on-demand virtual machines. We target these computational resources as representative of what is easily accessible for the general data science practitioner unlike DGX-2 that requires significant investment. We report results obtained from \ipoint{AWS}, Microsoft Azure and Stampede2. On Table \ref{tab:aws_azure_vs_stampede_specs}, we provide all relevant specifications for Azure and Stampede2 used in our experiments. \textcolor{blue}{Care was taken to select configurations on AWS and Azure to reasonably match the CPU as well as interconnect speeds of Stampede2. This allows rational assessment of performance of SciDDL across nearly similar platforms.} We present wall-clock time comparisons between \ipoint{AWS}, Azure and Stampede2 in section \ref{subsec:conventional_cloud} to determine the cluster to use for our large domain runs. In section \ref{subsec:strong_scaling}, we conduct strong scaling experiments for $128 \times 128$ and $256 \times 256$ domain sizes for 1 to 128 nodes (48 to 6144 cores) on Stampede2 to demonstrate scalability of our software. Finally, in section \ref{subsec:high_resolution_diffnet}, we present results for training a DiffNet model for \textbf{$512 \times 512$} and \textbf{$1024 \times 1024$} domain sizes for Burgers' inviscid equation (Eq.~\ref{eq:Inviscid_Burgers}) for parameter distributions characterizing the initial conditions (Eq.~\ref{eq:initial-condition}), which are currently not possible to train.

\begin{table}[!ht]
  \begin{center}
    \begin{tabular}{|c|c|c|c|}
    \hline
     {\bf Specification} & \ipoint{\bf AWS} & \shortstack{{\bf Azure}}  & {\bf Stampede2} \\
     \hline
     Type & \ipoint{\shortstack{Virtual \\Machine}} & \shortstack{Virtual \\ Machine} & Bare-Metal \\
     \hline
     CPU & \ipoint{\shortstack{Intel Xeon \\ Platinum 8000}} & \shortstack{Intel Xeon \\ Platinum 8168} & \shortstack{Intel Xeon \\ Platinum 8160} \\
     \hline
     CPU cores & \ipoint{72} & 44 & 48 \\
     \hline
     Memory (GB)& \ipoint{192} & 352& 192\\
     \hline
     Interconnect & \ipoint{\shortstack{Elastic \\ Fabric Adapter}} & \shortstack{EDR \\Infiniband} & \shortstack{Intel \\ Omni-Path} \\
     \hline
     Bandwidth & \ipoint{100 Gb/sec} & 100 Gb/sec & 100 Gb/sec \\
     \hline
     Topology & \ipoint{AWS Proprietary} & Fat tree & Fat tree \\
     \hline
\end{tabular}
\caption{Functional specifications of \ipoint{AWS}, Microsoft Azure and Stampede2 infrastructure used in our experiments. \label{tab:aws_azure_vs_stampede_specs}}
\end{center}
\end{table}

\subsection{Conventional HPC vs. Cloud Based HPC} 
\label{subsec:conventional_cloud}
In this section, we compare wall-clock times between \ipoint{AWS}, Microsoft Azure, and Stampede2 in order to determine the optimal HPC cluster configuration to train \emph{DiffNet} with very large ($1024\times 1024$) resolutions. On Table \ref{tab:aws_azure_vs_stampede}, we show per-epoch wall-clock times (in seconds) to train DiffNet with $64\times 64$ resolution using 1, 2 and 4 nodes. The total number of samples used for this experiment was $N_s = 4096$ and the global batch size was $b_s = 1024$; the number of processes per node was fixed at 4, with each process spawning 8 local threads. Single node performance on bare-metal Stampede2 is $\sim 2 \times$ faster than on Azure \ipoint{and AWS} VM. On the same table, we also compare per-epoch wall-clock times (in seconds) for different resolutions on 4 compute nodes (with 4 processes per node, 8 threads per process). Even though the infrastructure specifications of Azure, \ipoint{AWS} and Stampede2 are almost identical, slowness on Azure and \ipoint{AWS} can be attributed to the overheads associated with virtual machines.

\begin{table}[!ht]
  \begin{center}
    \begin{tabular}{|c|c|c|c|c|}
    \hline
     {\bf Domain Size} & {\bf Nodes} & \ipoint{\bf AWS} & {\bf Azure} & {\bf Stampede2}  \\
     \hline
     64x64 & 1 & \ipoint{131.0} & 113.1&67.2 \\
     \hline
     64x64 & 2 & \ipoint{65.2} & 54.9&34.9 \\
     \hline
     64x64 & 4 & \ipoint{32.4} & 28.6& 19.4\\
     \hline
     128x128 & 4& \ipoint{138.4} & 126.2 &68.5 \\
     \hline
     256x256 & 4 & \ipoint{650.5} & 597.6& 279.8\\
     \hline
\end{tabular}
\caption{Comparison of per-epoch wall-clock times (in seconds) between \ipoint{AWS}, Azure and Stampede2 for varying resolutions and different number of nodes (see Table \ref{tab:aws_azure_vs_stampede_specs} for cluster specs). For all three clusters, 4 processes were used per node (spawning 8 threads each). \label{tab:aws_azure_vs_stampede}}
\end{center}
\end{table}
\subsection{Scaling Experiments} 
\label{subsec:strong_scaling}
In Figure \ref{fig:sc_strong_scaling}, we report strong scaling results to train {\it DiffNet} for $128\times 128$ and $256\times 256$ resolutions, using from 4 to 128 nodes on Stampede2. In this experiment, we used 8 MPI processes per node and each process spawned 12 threads, to a total of 96 threads per node. This matches the full capacity of the Stampede2 Skylake nodes, which have 48 physical hyperthread-enabled CPU cores, resulting in 96 hardware threads per node. 
\textcolor{blue}{In Table \ref{tab:wall_clock_times}, we compare per-epoch wall clock time between a single GPU (Titan RTX as well as Tesla V100) with the wall clock time using 128 Stampede2 nodes. We show this (potentially unfair) comparison to illustrate the advantage of scale-up on CPUs using a distributed training approach}.

%, we show comparisons of wall clock times per epoch between GPU and Stampede2 using SciDDL. 
\begin{figure}[!ht]
  \centering
  \includegraphics[width=0.45\textwidth]{Figures/sc_strong_scaling.jpg}
  \caption{Strong scaling results for training {\it DiffNet} on Stampede2: per-epoch times (in seconds) versus number of nodes for $128\times 128$ and $256\times 256$ resolutions, using 8 processes per node and 12 threads per process.\label{fig:sc_strong_scaling}}
\end{figure}


\begin{table}[!ht]
  \begin{center}
    \begin{tabular}{|c|c|c|c|}
    \hline
     \thead{\bf Output \\ \bf resolution} &   \thead{\bf{1 Titan RTX} \\ \bf{(seconds)}} &   \thead{\ipoint{1 Tesla V100} \\\ipoint{(seconds)}} & \thead{\bf 128 Stampede2 nodes\\  \bf (seconds)} \\
     \hline
     128$\times$128 & 105 & \ipoint{130} & 4.6\\
     \hline
     256$\times$256	& 340 & \ipoint{494} & 12.7\\
     \hline
     512$\times$512	& 1401 & \ipoint{1961} & 25.3 \\
     \hline
     1024$\times$1024 & N/A & \ipoint{N/A}& 89.5 \\
     \hline
\end{tabular}
\caption{Comparison of per-epoch wall-clock time  between Titan RTX, \ipoint{Tesla V100} and SciDDL on 128 Stampede2 nodes to train Diffnet (of different resolutions) with 4096 samples. Training on large CPU clusters using SciDDL is $20-60\times$ faster than training on \textcolor{blue}{both GPU's. The 30-40\% change between the Titan RTX vs Tesla V100 is attributable to the 30\% difference in clockspeed between them.}\label{tab:wall_clock_times}}
\end{center}
\end{table}

% \begin{table}[!ht]
%   \begin{center}
%     \begin{tabular}{|c|c|c|c|}
%     \hline
%      {\bf Domain Size} &   {\bf FEM (seconds)} & {\bf SciDDL (seconds)} \\
%      \hline
%     %  128$\times$128 & 105 & 4.6\\
%     %  \hline
%     %  256$\times$256	& 340 & 12.7\\
%     %  \hline
%      512$\times$512	& 23.2 & 3.6 \\
%      \hline
%      1024$\times$1024 & 395.6 & 9.8 \\
%      \hline
% \end{tabular}
% \caption{Comparison of solve time for the finite element solution  and the inference time for the SciDDL solution \label{tab:comparison_FEM_ML}}
% \end{center}
% \end{table}

As discussed in section \ref{subsec:complexities}, our computation time complexity scales with $p$ and communication complexity is independent of $p$. In Figure \ref{fig:comp_vs_comm_wc_times_256x256_revised}, we show the computation and communication wall-clock times for different $p$. We observed that our communication times \textcolor{blue}{increase only slightly with $p$, as expected. Note that the communication times are significantly ($100\times$) smaller than compute times}.

\begin{figure}[!ht]
  \centering
  \includegraphics[width=0.45\textwidth]{Figures/comp_vs_comm_wc_times_256x256_revised.png}
  \caption{\textcolor{blue}{Computation and communication wall clock times for different $p$ corresponding to strong scaling results for domain size $256 \times 256$ in Figure \ref{fig:sc_strong_scaling}. Computation time decreases linearly with $p$, while communication time increases only slightly with $p$.} \label{fig:comp_vs_comm_wc_times_256x256_revised}}
\end{figure}

% \begin{figure}[!ht]
%   \centering
%   \includegraphics[width=0.45\textwidth]{Figures/loss_vs_epoch_128x128.png}
%   \caption{Loss vs. Epoch for 128x128 placeholder to demonstrate loss preservation independent of $p$ \label{fig:loss_vs_epoch_128x128}}
% \end{figure}
As discussed in section \ref{subsec:data_parallel_ddl}, the training samples are split in such a way as to guarantee loss decay integrity, i.e., the same exact problem is solved independently of the number of MPI processes. In Figure \ref{fig:loss_vs_epoch_256x256}, we show the loss vs. epoch for different values of $p$. The small deviation in loss values for different $p$ is due to rounding errors in \emph{MPI\_Allreduce} operations for computing gradient averages.

\begin{figure}[!ht]
  \centering
  \includegraphics[width=0.45\textwidth]{Figures/loss_vs_epoch_256x256.png}
  \caption{Comparison of loss decay vs. epoch for a subset of $p$ used in strong scaling experiments in Figure \ref{fig:sc_strong_scaling}. Loss decay is preserved (independent of $p$). \label{fig:loss_vs_epoch_256x256}}
\end{figure}

% \begin{figure}[!ht]
%   \centering
%   \includegraphics[width=0.45\textwidth]{Figures/loss_vs_epoch_error_256x256.png}
%   \caption{Maximum relative error in loss per epoch across for different $p$. These errors are bounded and are attributed to rounding errors in \emph{MPI\_Allreduce}. \label{fig:loss_vs_epoch_error_256x256}}
% \end{figure}
\begin{figure*}[ht]
\centering
\captionsetup{justification=centering}
    \begin{subfigure}{0.4\textwidth}
      \centering
      \subcaption*{SciDDL solution}
      \includegraphics[trim=80 50 80 80,clip,width=1.0\linewidth]{Figures/comparison_images/ml-m1024-c03.png}
    %   \caption{}
    %   \label{fig:ST-Diff3D}
    \end{subfigure}
    %\\
    \begin{subfigure}{0.4\textwidth}
      \centering
      \subcaption*{Finite element solution}
      \includegraphics[trim=80 50 80 80,clip,width=1.0\linewidth]{Figures/comparison_images/fe-m1024-c3.png}
    %   \caption{}
    %   \label{fig:ST-Adv3D}
    \end{subfigure}
    \caption{Inviscid Burgers' equation  solved on $1024\times1024$ pixels (left) or elements (right)}
    \label{fig:comparison-panel_1024}
\end{figure*}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.45\textwidth]{Figures/loss_1024.jpg}
  \caption{Loss vs. epoch for training DiffNet with domain size $1024\times 1024$ on Stampede2 using 256 sample points and batch size 64.\label{fig:loss_1024}} \vspace{-0.2in}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.45\textwidth]{Figures/loss_512.jpg}
  \caption{Loss vs. epoch for training DiffNet with domain size $512\times 512$ on Stampede2 using 256 sample points and batch size 64.\label{fig:loss_512}}\vspace{-0.2in}
\end{figure}

\begin{figure}[!ht]
    \centering
    \begin{minipage}[t]{.4\textwidth}
      \centering
      \begin{tikzpicture}
      \begin{axis}[
          width=0.99\linewidth, % Scale the plot to \linewidth
          %grid=major, % Display a grid
          %grid style={line width=.1pt, draw=gray!50}, % Set the style
          xlabel=$x$, % Set the labels
          ylabel=$u$,
          legend cell align={left},
          legend style={at={(1,0)},anchor=south east,legend columns=1}, % Put the legend below the plot
          grid=both,
          x tick label style={rotate=0,anchor=north} % Display labels sideways
        ]
         \addplot+ [color=black,mark=none,line width=1.2pt]
        table[x expr={\thisrow{"arc_length"}},y expr={\thisrow{"u_ml"}},col sep=comma]{Data/solution_plots/line_cuts/n_512_c_10.csv};
        \addplot+ [color=red,mark=none]
        table[x expr={\thisrow{"arc_length"}},y expr={\thisrow{"u_fem"}},col sep=comma]{Data/solution_plots/line_cuts/n_512_c_10.csv};
        \addplot+ [color=blue,dashed,mark=none,line width=1pt]
        table[x expr={\thisrow{"arc_length"}},y expr={\thisrow{"u_fdm"}},col sep=comma]{Data/solution_plots/line_cuts/n_512_c_10.csv};
        \legend{\scriptsize{SciDDL}, \scriptsize{FEM, space-time},\scriptsize{FDM, time-marching}}
      \end{axis}
    \end{tikzpicture}
    \end{minipage}
    \caption{\textcolor{blue}{An example of the solution profile $u$ vs. $x$ at the final time ($t = 0.2$), compared for different methods. Resolution = $512\times 512$ and $c = 10$}}
    \label{fig:plot-solutions-vs-x-t-1-resolution-512-c-10}
\end{figure}


%\vspace{-0.3in}
\subsection{High Resolution DiffNet} 
\label{subsec:high_resolution_diffnet}
In this sub-section, we illustrate the ability of the framework to train {\it DiffNet} models with very high resolution outputs (sizes $\ge 512\times 512$). This typically requires $\ge 2000$ epochs until convergence (for different ranges of the initial condition frequency $c$) \textcolor{blue}{using a first-order optimizer like SGD}.

{\bf Example 1:} In the first example, we train a DiffNet to produce outputs of resolution $1024 \times 1024$. We emphasize that generative models of this size have hitherto fore not been trained (to the best of our knowledge). We train the DiffNet to be predictive in a range of the parameter $c\in [3,6]$. We remind the reader that $c$ represents a one-parameter family of initial conditions to the inviscid Burgers equation. The training sample set consists of 256 points from $c\in [3,6]$. We set the mini-batch size to 64. This model was trained on 8 nodes of Stampede2 (with 8 processes per node), taking 2200 epochs till convergence (see Fig.~\ref{fig:loss_1024}). The runtime for this training was 32 hours. 

After training, we performed inference using the DiffNet for a set of initial conditions from the one-parameter family. Results for $c = 3$ are shown in Fig.~\ref{fig:comparison-panel_1024}, where we compare the DiffNet inference result with the solution from an optimized FEM solver (based on the Petsc library) of the inviscid Burgers equation. While the general trend of the solution (as the wave evolves -- from left to right in the figures -- and forms shocks) is captured well, there is still room for improvement as the more diffused nature of the ML solution indicates. We hypothesize that using higher order Sobel filters (i.e. computing the gradients using higher order stencils) could help in eliminating the diffusive features of the ML solution. We continue to explore these aspects. 


% Results for $1024\times 1024$ resolution: 256 training examples, mini-batch size 64, $c\in [3,6]$; 64 processes, 8 nodes (Stampede2); ran to 2200 epochs (32hrs runtime).

% \begin{figure}[!ht]
%   \centering
%   \includegraphics[width=0.45\textwidth]{Figures/result_1024_c_3.jpg}
%   \caption{Inviscid Burgers' solution for $1024\times 1024$ and $c=3$ \label{fig:result_1024_c_3}}
% \end{figure}

% \begin{figure}[!ht]
%   \centering
%   \includegraphics[width=0.45\textwidth]{Figures/result_1024_c_3_3D.jpg}
%   \caption{Inviscid Burgers' solution for $1024\times 1024$ and $c=3$ \label{fig:result_1024_c_3_3D}}
% \end{figure}


{\bf Example 2:} In the second example, we explore if the DiffNet can be trained to predict solutions for a much larger distribution of the initial conditions. We train a DiffNet to predict solutions at $512\times 512$ resolution, but for initial conditions from $c\in [3,16]$. At higher values of c (which represent initial conditions exhibiting higher frequencies), we expect the formation of multiple shocks. The traditional numerical solutions for these initial conditions have to be carefully performed. We set the mini-batch size to 64. This model was trained on 8 nodes (64 processors) on Stampede2, taking 4000 epochs till convergence (see Fig.~\ref{fig:loss_512}). The runtime for training this model was 15 hours. Notice that the loss in this case is significantly larger than the previous example. This is due to two reasons: the reduced resolution ($1024 \rightarrow 512$) and, more importantly, the larger $c$ space.  

After training, we again performed inference using the DiffNet for a set of initial conditions from the one-parameter family. Results for $c = 3, 5, 10, 13$ are shown in Fig.~\ref{fig:comparison-panel}, where we compare the DiffNet inference result with the solution from an optimized FEM solver (based on the Petsc library) of the inviscid Burgers equation. As before, the general trend of the solution (as the wave evolves -- from left to right in the figures -- and forms shocks) is captured well, but there is still room for improvement. 

\textcolor{blue}{Fig.~\ref{fig:plot-solutions-vs-x-t-1-resolution-512-c-10} and Table~\ref{tab:norms-solutions-and-differences} show additional, quantitative comparison  between the DiffNet results with a stabilized Finite Element solution (at $512 \times 512$ resolution) against a very high resolution ($2048 \times 2048$) finite difference solution. Fig.~\ref{fig:plot-solutions-vs-x-t-1-resolution-512-c-10} plots the solution at one time point ($t=0.2$), and suggests that stabilized finite element space-time approach is still unable to capture the shocks, while the DiffNet is able to accurately capture the shock without any dispersive effects. This is particularly promising as the loss function used in the DiffNet is the simplest one possible, with significant room for improvement. Table~\ref{tab:norms-solutions-and-differences} shows the L2 error norm (in space-time) of the DiffNet and FEM solution against the high resolution FDM solution. Interestingly, we find that the DiffNet approach produces more accurate results for initial conditions exhibiting more waves (larger c). This is in contrast to what is observed in traditional approaches (compare the last two columns of Table~\ref{tab:norms-solutions-and-differences}).} We find it promising that the DiffNet is able act as a general PDE solver for a wide range of initial conditions. This strongly suggests that, with the proper training infrastructure, it is possible to develop truly general PDE solvers that produce accurate solutions for general classes of PDE's. 

\begin{table}[]
    \centering
    \color{blue}{
\csvreader[
  tabular=|c|c|c|c|c|c|c|,
  table head=\hline \bfseries{$N$} & \bfseries{$c$} & \bfseries{$||u_g||_2$} & \bfseries{$||u_{fd}||_2$} & \bfseries{$||u_{fe}||_2$} & \bfseries{$||\delta^{g}_{fd}||_2$} & \bfseries{$||\delta^{fe}_{fd}||_2$} \\ \hline,
  late after last line=\\ \hline % horizontal line at the end of the table
]{
  Data/solution_norms/norms_table.csv
}{}{\csvlinetotablerow}
}
    \caption{\textcolor{blue}{Norm of different solutions (denoted $u$) and their differences (denoted $\delta$). $u_g$ is the solution generated through SciDDL, $u_{fd}$ is the solution obtained using explicit time marching with finite difference approximation; and $u_{fe}$ is the ``space-time" solution  obtained through finite element approximation in \textit{both} space and time. The differences between them: $\delta^{g}_{fd} = u_g - u_{fd}$ and $\delta^{fe}_{fd} = u_{fe} - u_{fd}$. All norms are calculated over the entire spatiotemporal domain}}
    \label{tab:norms-solutions-and-differences} %\vspace{-0.2in}
\end{table}

\textcolor{blue}{{\bf Effect of batch size on solution using first order (SGD) and second order (L-BFGS) optimizers:} The data parallelism afforded by SciDDL potentially allows one to use larger batch sizes. However, it is well known that increasing batch sizes can decrease the convergence of Stochastic Gradient Descent (SGD). We explore this effect of batch size on the training performance. Fig.~\ref{fig:loss-epoch-plots-64x64}(top) plots evolution of the loss function with training epochs for increasing batch size (BS) for a $64 \times 64$ resolution DiffNet. We clearly see some degradation in convergence rate as the batch size is increased to 64. We next trained the same network using a second order optimizer (L-BFGS) implemented in the SciDDL framework. Fig~\ref{fig:loss-epoch-plots-64x64}(bottom) shows negligible impact of increasing batch size on convergence. As expected, the second order method converges in fewer epochs, with similar reduction in loss happening within 10 training epochs as compared to 150 epochs for SGD. L-BFGS optimizers require larger memory (to evaluate the Hessian) which a distributed approach (like SciDDL or LBANN) can gracefully accommodate.}


\begin{figure}[!ht]
    \centering
    \begin{minipage}{.49\textwidth}
  \begin{center}
  \begin{tikzpicture}
      \begin{axis}[
    %   xmode=log,
    %   ymode=log,
    %   log ticks with fixed point,
          width=0.99\linewidth, % Scale the plot to \linewidth
          height=4cm,
          xlabel={Epoch}, % Set the labels
          ylabel=$\log_{10}(L)$, % Set the labels
          legend style={at={(0.95,0.95)},anchor=north east,legend columns=2}, % Put the legend below the plot
        %   xmin=0,
        %   xmax=200,
          ymin=-0.7,
          ymax=1.5,
          grid=both,
          x tick label style={rotate=0,anchor=north}
        ]
        \addplot+ [mark=none,line width=1pt]
        table[x expr={(\thisrowno{1})},y expr={log10(\thisrowno{3})},col sep=space]{Data/batch_size_experiment/n-0064/sgd/log_processed_bs_8.txt};
        \addplot+ [mark=none,line width=1pt]
        table[x expr={(\thisrowno{1})},y expr={log10(\thisrowno{3})},col sep=space]{Data/batch_size_experiment/n-0064/sgd/log_processed_bs_16.txt};
        \addplot+ [mark=none,line width=1pt]
        table[x expr={(\thisrowno{1})},y expr={log10(\thisrowno{3})},col sep=space]{Data/batch_size_experiment/n-0064/sgd/log_processed_bs_32.txt};
        \addplot+ [mark=none,line width=1pt]
        table[x expr={(\thisrowno{1})},y expr={log10(\thisrowno{3})},col sep=space]{Data/batch_size_experiment/n-0064/sgd/log_processed_bs_64.txt};
        % \addplot+
        % table[x expr={(\thisrow{nodes})},y expr={\thisrow{L2_Err}},col sep=space]{results_data/case_7_diff_gaussian_adref/k_1e-2_etol_1e-4/case7_error_data_adref.txt};
        \legend{\scriptsize{BS=8}, \scriptsize{BS=16}, \scriptsize{BS=32}, \scriptsize{BS=64}}
      \end{axis}
    \end{tikzpicture}
    \subcaption{SGD}
    \label{fig:64x64-sgd-loss-epoch}
    \end{center}
    \end{minipage}
    \\
    \begin{minipage}{.49\textwidth}
  \begin{center}
  \begin{tikzpicture}
      \begin{axis}[
    %   xmode=log,
    %   ymode=log,
    %   log ticks with fixed point,
          width=0.99\linewidth, % Scale the plot to \linewidth
          height=4cm,
          xlabel={Epoch}, % Set the labels
          ylabel=$\log_{10}(L)$, % Set the labels
          legend style={at={(0.95,0.95)},anchor=north east,legend columns=2}, % Put the legend below the plot
          %   xmin=0,
        %   xmax=200,
          ymin=-0.7,
          ymax=1.5,
          grid=both,
          x tick label style={rotate=0,anchor=north}
        ]
        \addplot+ [mark=none,line width=1pt]
        table[x expr={(\thisrowno{1})},y expr={log10(\thisrowno{3})},col sep=space]{Data/batch_size_experiment/n-0064/lbfgs/log_processed_bs_8.txt};
        \addplot+ [mark=none,line width=1pt]
        table[x expr={(\thisrowno{1})},y expr={log10(\thisrowno{3})},col sep=space]{Data/batch_size_experiment/n-0064/lbfgs/log_processed_bs_16.txt};
        \addplot+ [mark=none,line width=1pt]
        table[x expr={(\thisrowno{1})},y expr={log10(\thisrowno{3})},col sep=space]{Data/batch_size_experiment/n-0064/lbfgs/log_processed_bs_32.txt};
        \addplot+ [mark=none,line width=1pt]
        table[x expr={(\thisrowno{1})},y expr={log10(\thisrowno{3})},col sep=space]{Data/batch_size_experiment/n-0064/lbfgs/log_processed_bs_64.txt};
        % \addplot+
        % table[x expr={(\thisrow{nodes})},y expr={\thisrow{L2_Err}},col sep=space]{results_data/case_7_diff_gaussian_adref/k_1e-2_etol_1e-4/case7_error_data_adref.txt};
        \legend{\scriptsize{BS=8}, \scriptsize{BS=16}, \scriptsize{BS=32}, \scriptsize{BS=64}}
      \end{axis}
    \end{tikzpicture}
    \subcaption{L-BFGS}
    \label{fig:64x64-lbfgs-loss-epoch}
    \end{center}
    \end{minipage}
  \caption{\textcolor{blue}{Loss vs. epoch for $64\times 64$ domain DiffNet with varying batch-size (BS). Second order optimizers (L-BFGS) provide minimal convergence drift with higher batch-size. All training done on 1 node of Nova}}
    \label{fig:loss-epoch-plots-64x64}
\end{figure}


\textcolor{blue}{The increased computational overhead results in increased time per epoch, and this is plotted in Fig.~\ref{fig:loss-time-plots-64x64}. While L-BFGS takes an order of magnitude less number of epochs to converge, each epoch is more expensive due to memory and compute requirements from evaluating the Hessian. It is informative also to look at the results in terms of computational time to reach a certain convergence threshold, with L-BFGS schemes about $3 \times$ faster than the SGD scheme. This reduction in computational time to reach a desired loss threshold can be enhanced via parallelization. SciDDL allows parallelization of L-BFGS based training across multiple CPU nodes, and this training across multiple nodes proportionally decreases the time-to-train, as shown in Table~\ref{tab:128x128-lbfgs-scaling-nova}}

\begin{table}[]
    \centering
    \ipoint{
\csvreader[
  tabular=|c|c|c|,
  table head=\hline 
  \bfseries{$p$} & \bfseries{$64 \times 64$} & \bfseries{$128 \times 128$} 
  \\ \hline,
  late after last line=\\ \hline % horizontal line at the end of the table
]{
  Data/scaling_experiment_nova/lbfgs_100_epochs_combined_064_128_minute.txt
}{}{\csvlinetotablerow}
}
    \caption{\textcolor{blue}{Time (in minutes) taken to complete $100$ epochs of the L-BFGS method for the $64\times 64$ and $128\times 128$ domain DiffNet on different number of processors}}
    \label{tab:128x128-lbfgs-scaling-nova} \vspace{-0.2in}
\end{table}

\textcolor{blue}{These results are very promising as they allow using second order methods -- which are less sensitive to large batch sizes -- and data parallelization to reduce time-to-solve to beat SGD based approaches. We include additional results in the appendix A.}

\begin{figure}[!ht]
    \centering
    \begin{minipage}{.49\textwidth}
  \begin{center}
  \begin{tikzpicture}
      \begin{axis}[
    %   xmode=log,
    %   ymode=log,
    %   log ticks with fixed point,
          width=0.99\linewidth, % Scale the plot to \linewidth
          height=4cm,
          xlabel={time (sec)}, % Set the labels
          ylabel=$\log_{10}(L)$, % Set the labels
          legend style={at={(0.95,0.95)},anchor=north east,legend columns=2}, % Put the legend below the plot
          %   xmin=0,
        %   xmax=200,
          ymin=-0.7,
          ymax=1.5,
          grid=both,
          x tick label style={rotate=0,anchor=north}
        ]
        \addplot+ [mark=none,line width=1pt]
        table[x expr={(\thisrowno{0})},y expr={log10(\thisrowno{3})},col sep=space]{Data/batch_size_experiment/n-0064/sgd/log_processed_bs_8.txt};
        \addplot+ [mark=none,line width=1pt]
        table[x expr={(\thisrowno{0})},y expr={log10(\thisrowno{3})},col sep=space]{Data/batch_size_experiment/n-0064/sgd/log_processed_bs_16.txt};
        \addplot+ [mark=none,line width=1pt]
        table[x expr={(\thisrowno{0})},y expr={log10(\thisrowno{3})},col sep=space]{Data/batch_size_experiment/n-0064/sgd/log_processed_bs_32.txt};
        \addplot+ [mark=none,line width=1pt]
        table[x expr={(\thisrowno{0})},y expr={log10(\thisrowno{3})},col sep=space]{Data/batch_size_experiment/n-0064/sgd/log_processed_bs_64.txt};
        % \addplot+
        % table[x expr={(\thisrow{nodes})},y expr={\thisrow{L2_Err}},col sep=space]{results_data/case_7_diff_gaussian_adref/k_1e-2_etol_1e-4/case7_error_data_adref.txt};
        \legend{\scriptsize{BS=8}, \scriptsize{BS=16}, \scriptsize{BS=32}, \scriptsize{BS=64}}
      \end{axis}
    \end{tikzpicture}
    \subcaption{SGD}
    \label{fig:64x64-sgd-loss-time}
    \end{center}
    \end{minipage}
    \\
    \begin{minipage}{.49\textwidth}
  \begin{center}
  \begin{tikzpicture}
      \begin{axis}[
    %   xmode=log,
    %   ymode=log,
    %   log ticks with fixed point,
          width=0.99\linewidth, % Scale the plot to \linewidth
          height=4cm,
          xlabel={time (sec)}, % Set the labels
          ylabel=$\log_{10}(L)$, % Set the labels
          legend style={at={(0.95,0.95)},anchor=north east,legend columns=2}, % Put the legend below the plot
          %   xmin=0,
        %   xmax=200,
          ymin=-0.7,
          ymax=1.5,
          grid=both,
          x tick label style={rotate=0,anchor=north}
        ]
        \addplot+ [mark=none,line width=1pt]
        table[x expr={(\thisrowno{0})},y expr={log10(\thisrowno{3})},col sep=space]{Data/batch_size_experiment/n-0064/lbfgs/log_processed_bs_8.txt};
        \addplot+ [mark=none,line width=1pt]
        table[x expr={(\thisrowno{0})},y expr={log10(\thisrowno{3})},col sep=space]{Data/batch_size_experiment/n-0064/lbfgs/log_processed_bs_16.txt};
        \addplot+ [mark=none,line width=1pt]
        table[x expr={(\thisrowno{0})},y expr={log10(\thisrowno{3})},col sep=space]{Data/batch_size_experiment/n-0064/lbfgs/log_processed_bs_32.txt};
        \addplot+ [mark=none,line width=1pt]
        table[x expr={(\thisrowno{0})},y expr={log10(\thisrowno{3})},col sep=space]{Data/batch_size_experiment/n-0064/lbfgs/log_processed_bs_64.txt};
        % \addplot+
        % table[x expr={(\thisrow{nodes})},y expr={\thisrow{L2_Err}},col sep=space]{results_data/case_7_diff_gaussian_adref/k_1e-2_etol_1e-4/case7_error_data_adref.txt};
        \legend{\scriptsize{BS=8}, \scriptsize{BS=16}, \scriptsize{BS=32}, \scriptsize{BS=64}}
      \end{axis}
    \end{tikzpicture}
    \subcaption{L-BFGS}
    \label{fig:64x64-lbfgs-loss-time}
    \end{center}
    \end{minipage}
      \caption{\textcolor{blue}{Loss vs. time to solve for $64\times 64$ domain DiffNet with varying batch-size (BS). Second order optimizers (L-BFGS) are substantially slower than SGD. All training done on 1 node of Nova}}
    \label{fig:loss-time-plots-64x64}
\end{figure}


{\bf Comparison of run-times between DiffNet and FEM based solutions}: While the training times for ML models is admittedly long, once trained, the inference step is often very fast. This allows one to amortize the cost of training across multiple users and instances. The availability of a general 'NeuralPDE' makes this a viable possibility. We quantify this argument by comparing the time it takes for a trained DiffNet to make a prediction (i.e. inference) with the time it takes for a well optimized FEM solver to perform the same prediction. \textcolor{blue}{Both DiffNet inference and FEM solve are performed on one node of Stampede2.} This comparison is reported in Table~\ref{tab:comparison_FEM_ML}, which shows a 40x improvement in prediction time. We emphasize that the inference step is not optimized, suggesting that the 40x improvement we show is a lower bound. 

\begin{table}[!ht]
  \begin{center}
    \begin{tabular}{|c|c|c|c|}
    \hline
     {\bf Domain Size} &   {\bf FEM (seconds)} & {\bf SciDDL (seconds)} \\
     \hline
    %  128$\times$128 & 105 & 4.6\\
    %  \hline
    %  256$\times$256	& 340 & 12.7\\
    %  \hline
     512$\times$512	& 23.2 & 3.6 \\
     \hline
     1024$\times$1024 & 395.6 & 9.8 \\
     \hline
\end{tabular}
\caption{Comparison of solve time for the finite element solution  and the inference time for the SciDDL solution \label{tab:comparison_FEM_ML}}
\end{center}
\end{table}



\section{Conclusions}
In this work, we report on a data distributed computing approach for training large neural network architectures, especially in the context of data-free generative models that serve as PDE solvers. We  highlighted  some of the key challenges and improvements over conventional GPU based training strategies, as well as other data-parallel approaches. We demonstrated excellent scaling  results  for  our  framework  on current  supercomputers. We illustrated the ability of this framework to enable practitioners to train very large models, thus enabling practical applications of such 'neuralPDE' solvers. We  believe  that availability of tools like the one presented here will help democratize the ability of a data scientist to produce (near) real time predictions of complex systems characterized by PDEs. Our future goals include extension of the framework to incorporate model parallelism for increased scaleup, as well as apply second order strategies to train DiffNets for a wide range of PDE's. 

\clearpage
% \csvautotabular{Data/solution_norms/norms_table.csv}

% \csvreader[
%   tabular=|c|c|c|c|c|c|c|,
%   table head=\hline \bfseries{Name} & \bfseries{Given Name} & \bfseries{Matriculation} & \bfseries{Gender} & \bfseries{Grade} \\ \hline,
%   late after last line=\\ \hline % horizontal line at the end of the table
% ]{
%   Data/solution_norms/norms_table.csv
% }{}{\csvlinetotablerow}



\begin{figure*}[!ht]
\centering
\captionsetup{justification=centering}
    \begin{subfigure}{0.4\textwidth}
      \centering
      \subcaption*{SciDDL solution}
      \includegraphics[trim=30 0 0 30,clip,width=1.0\linewidth]{Figures/comparison_images/small/ml-m512-c03-small.png}
    %   \caption{}
    %   \label{fig:ST-Diff3D}
    \end{subfigure}
    %\\
    \begin{subfigure}{0.4\textwidth}
      \centering
      \subcaption*{Finite element solution}
      \includegraphics[trim=30 0 0 30,clip,width=1.0\linewidth]{Figures/comparison_images/small/fe-m512-c03-small.png}
    %   \caption{}
    %   \label{fig:ST-Adv3D}
    \end{subfigure}
    \\
    \begin{subfigure}{.4\textwidth}
      \centering
      \includegraphics[trim=30 0 0 30,clip,width=1.0\linewidth]{Figures/comparison_images/small/ml-m512-c05-small.png}
    %   \caption{}
    %   \label{fig:ST-AC3D}
    \end{subfigure}
    %\\
    \begin{subfigure}{.4\textwidth}
      \centering
      \includegraphics[trim=30 0 0 30,clip,width=1.0\linewidth]{Figures/comparison_images/small/fe-m512-c05-small.png}
    %  \caption{}
    %   \label{fig:ST-Diff-slice}
    \end{subfigure}
    \\
    \begin{subfigure}{.4\textwidth}
      \centering
      \includegraphics[trim=30 0 0 30,clip,width=1.0\linewidth]{Figures/comparison_images/small/ml-m512-c10-small.png}
    %   \caption{}
    %   \label{fig:ST-Adv-slice}
    \end{subfigure}
    %\\
    \begin{subfigure}{.4\textwidth}
      \centering
      \includegraphics[trim=30 0 0 30,clip,width=1.0\linewidth]{Figures/comparison_images/small/fe-m512-c10-small.png}
    %   \caption{}
    %   \label{fig:ST-AC-slice}
    \end{subfigure}
    \\
    \begin{subfigure}{.4\textwidth}
      \centering
      \includegraphics[trim=30 0 0 30,clip,width=1.0\linewidth]{Figures/comparison_images/small/ml-m512-c13-small.png}
    %   \caption{}
    %   \label{fig:ST-Adv-slice}
    \end{subfigure}
    %\\
    \begin{subfigure}{.4\textwidth}
      \centering
      \includegraphics[trim=30 0 0 30,clip,width=1.0\linewidth]{Figures/comparison_images/small/fe-m512-c13-small.png}
    %   \caption{}
    %   \label{fig:ST-AC-slice}
    \end{subfigure}
    \caption{Contour plots of the solution to the inviscid Burgers' equation: solutions from DiffNet (left) vs solutions from a finite element solver (right). The initial condition is characterized by the wave number $c$ (defined in \ref{eq:initial-condition}). The first row presents solution for $c = 3$ and subsequently for $c$ = 5, 10 and 13 in the latter rows respectively. On the left, the image size is $512\times512$ pixels, whereas on the right, the discretization is a mesh of $512\times512$ bilinear quadrilateral elements.}
    \label{fig:comparison-panel}
\end{figure*}
\clearpage




==> previous_work/algo_development.tex <==
GPUs remain the overwhelmingly popular compute platform for training these models. GPU memory utilization during training is driven by three factors: 1) number of model parameters in the network, 2) mini-batch size, and 3) size of intermediate tensors created during loss and gradient computations. A known limitation of GPUs is their relatively small available memory: for example, a state-of-the-art NVIDIA Tesla V100 GPU has only 32GB memory. Peak memory utilization to train a DiffNet for domain size $512 \times 512$ and mini-batch size 64 is $\sim$64GB, which is twice the available GPU memory. Due to these memory limitations, training on GPUs is done using mini-batches as small as 16, which in turn results in slow convergence and prohibitive wall-clock times. On Table \ref{tab:gpu_runtimes_memory}, we show maximum batch size and GPU memory utilization for different domain sizes that we were able to train on a NVIDIA Tesla RTX with 24GB memory. \textit{DiffNet training on domain sizes $> 512 \times 512$ is not feasible on currently available GPUs including Tesla V100}.
 \begin{table}[!ht]
  \begin{center}
    \begin{tabular}{|c|c|c|c|}
    \hline
     {\bf Domain Size} &  {\bf Batch Size} & {\bf GPU Memory (GB)} & {\bf Time/Epoch (s)}\\
     \hline
     128$\times$128 & 16	& 0.7 & 105\\
     \hline
     256$\times$256	& 16	& 2.1 & 340\\
     \hline
     512$\times$512	& 16	& 16.4 & 1401\\
     \hline
\end{tabular}
\caption{GPU  memory utilization and time per epoch for 4096 samples for different domain and batch sizes. On Titan RTX with 24GB memory, Diffnet training on domain sizes $> 512 \times 512$ with batch size 16 is not feasible. \label{tab:gpu_runtimes_memory}}
\end{center}
\end{table}

NVIDIA AI Servers like DGX-2 can accommodate bigger batch sizes by distributing the batches across multiple GPUs in a single unit with more cumulative GPU memory (256GB with 8 GPUs and 32GB/GPU). However, they come with an expensive price tag of $\sim$\$0.5M and are not affordable for the general practitioner. In spite of this price tag, the maximum available memory \textbf{is still the same} as the cumulative memory available on 1 or 2 nodes of a CPU cluster.
 
In order to overcome those memory limitations, our \emph{SciDDL} framework is based on \emph{data parallel} distributed training on multi-node CPU clusters with 5-10x more memory-per-node than a single GPU, and multiple cores-per-node connected via high-end interconnects with low latency and high bandwidth, which can match or exceed the performance of GPUs. The rest of this section is organized as follows: in section \ref{subsec:data_parallel_ddl} we provide details on data parallel training; in section \ref{subsec:sync_bn} we discuss the need for synchronized batch normalization; the OpenMP and MPI based hybrid distribution model is explained in section \ref{subsec:hybrid_distribution_model}; time complexities for computation and communication are discussed in section \ref{subsec:complexities}, and a comparison to open-source software is made in section \ref{subsec:comparison_to_oss}. In Table \ref{tab:notations}, we summarize the notations used in this section. 

\begin{table}[!ht]
  \begin{center}
    \begin{tabular}{|cc|}
    \hline
     $N_s$ & Total number of samples \\
     $b_s$ & Number of samples in a mini-batch \\
     $N_s^{loc}$ & Local number of samples \\
     $b_s^{loc}$ & Local mini-batch size \\
     $N_b$ & Number of mini-batches \\
     $N_w$ & Number of weights in the model \\
     $p$   & Number of MPI tasks in \emph{comm} \\
     $N_t$ & Number of threads per MPI task \\
     $F$   & Forward propagation complexity \\
     $B$   & Backward propagation complexity \\
     $L$   & Loss function \\
     $\theta$ & Model parameters \\
     $G_\theta$ & Gradient w.r.t model parameters \\
     \hline
\end{tabular}
\caption{Notations used in this section \label{tab:notations}}
\end{center}
\end{table}

\subsection{Data Parallel Distributed Deep Learning}
\label{subsec:data_parallel_ddl}
We use the {\it data parallel} strategy, where multiple replicas of a model are simultaneously trained to optimize a single objective function \cite{bennun_parallel_dnn}. In this approach, the training mini-batches are equally split among the available workers, as shown in Figure \ref{fig:dl_parallel}. Each of these workers asynchronously perform forward and back-propagation of their local mini-batch through the neural network. After each mini-batch, the locally computed gradients are averaged among workers via an {\it MPI\_Allreduce} operation, and that average is used by each local optimizer to update the layer parameters. The loss function is also computed locally, and the objective value is averaged among workers.
\begin{figure}[!ht]
  \centering
  \includegraphics[width=0.48\textwidth]{Figures/dl_dataparallel.png}
  \caption{Data Parallel Deep-Learning : multiple replicas of the model are asynchronously trained by workers, each worker using a subset of the global mini-batch. \label{fig:dl_parallel}}
\end{figure}

It is important that the samples (training examples) are split among workers in such a way that the same exact problem gets solved no matter the number of processes (MPI ranks). For that purpose, we adjust the total number of samples $N_s$ and the batch size $b_s$ to make them divisible by the number of workers $p$, such that the {\it local} sample count and batch size are given by
\begin{eqnarray}
N_s^{loc} = \ceil{\frac{N_s}{p}}, \\
b_s^{loc} = \floor{\frac{b_s}{p}}.
\end{eqnarray}
Furthermore, as shown in Figure \ref{fig:mini_batch_split}, each worker draws their local mini-batch sequentially from the global sample pool, in such a way that their union ({\it global} mini-batch) would equal the one used in a single-processor run with the same values of $N_s$ and $b_s$. This guarantees exactly identical results (modulo rounding errors due to gradient reduction) for any number of workers used. Finally, one can easily show that, when $N_s$ is not divisible by $b_s$, the remainder $N_s\mod b_s$ will still be divisible by $p$, which enforces optimal load balancing by guaranteeing that the local mini-batches processed by each worker at any given time have identical sizes.
\begin{figure}[!ht]
  \centering
  \includegraphics[width=0.48\textwidth]{Figures/mini_batch_split.png}
  \caption{Data splitting across workers in a parallel run: mini-batches are always guaranteed to have the same size across workers at any given time, promoting optimal load balance.\label{fig:mini_batch_split}}
\end{figure}

Algorithm \ref{alg:dl_parallel_algo} summarizes our per-epoch strategy for distributed training using the data parallel paradigm.
\begin{algorithm}[H]
%\KwResult{One epoch using data parallel training}
Generate $p N_s^{loc}$ samples, split in mini-batches of size $b_s^{loc}$\\
\For{$mb = 1$ \KwTo $N_b$} {
   {\bf x}_i \gets \{$b_s^{loc}$ samples\}                  \Comment{Worker $i$ local mini-batch}
   \ell_i(\theta) \gets L({\bf x}_i, G_\theta(\rvb, \nu))   \Comment{Forward pass and local loss}
   {\bf g}_i(\theta) \gets \nabla\ell_i(\theta)             \Comment{Back-prop and local gradient}
   \ell(\theta) \gets \frac{1}{p} \sum \ell_i(\theta)       \Comment{Average loss using MPI\_Allreduce}
   {\bf g}(\theta) \gets \frac{1}{p} \sum {\bf g}_i(\theta) \Comment{Average grad using MPI\_Allreduce}
   \Delta\theta \gets u({\bf g}, \theta, t)                 \Comment{Run local optimizer}\\
   \theta \gets \theta + \Delta\theta                       \Comment{Update network parameters}
}
\caption{Data parallel distributed deep learning (1 epoch)\label{alg:dl_parallel_algo}}
\end{algorithm}

\subsection{Synchronized Batch-normalization}
\label{subsec:sync_bn}
Batch Normalization (BN) is a procedure that dramatically improves the convergence of neural networks by re-scaling and re-centering data using running statistics, namely mean and variance, accumulated from each mini-batch in the course of an epoch \cite{ioffe_batchnorm}. This creates a dependency on the local mini-batch size, breaking the paradigm of problem independence on the number of workers discussed in section \ref{subsec:data_parallel_ddl}.
To remove this dependency, we developed a scheme to synchronize the mean and variance statistics at all BN layers by performing an {\it MPI\_Allreduce} operation after each epoch. This is especially important when the local mini-batch size on each processor is small, which would result in poor statistics and have a negative impact on validation accuracy. The BN synchronization scheme is explained in Algorithm \ref{alg:dl_bn_sync}.

\begin{algorithm}[H]
\ForEach{$\textrm{epoch}$} {
\ForEach{$\textrm{BN layer in network}$} {
\If{\textrm{in evaluation}} {
   \mu_{\mathcal{B}} \gets \frac{1}{p} \sum_i^p \mu_{\mathcal{B}}^{(i)} \Comment{Allreduce BN means}
   \sigma_{\mathcal{B}}^2 \gets \frac{1}{p} \sum_i^p {\sigma_{\mathcal{B}}^2}^{(i)} \Comment{Allreduce BN variances}
}}}
\caption{Batch-normalization synchronization algorithm\label{alg:dl_bn_sync}}
\end{algorithm}

\subsection{Hybrid Distribution Model}
\label{subsec:hybrid_distribution_model}
Our parallel distribution scheme is based on the so called {\it hybrid} MPI-OpenMP programming paradigm, in which communication between processes is done via MPI, while each process can spawn its own OpenMP threads that run inside a single shared-memory processor (SMP) node, as illustrated in Figure \ref{fig:hybrid_distribution}. Furthermore, since the OpenMP threads only communicate with other threads within the same SMP node, and MPI routines are only invoked outside of OpenMP parallel regions, our distribution scheme can be said to model the {\it process-to-process} hybrid paradigm.
In particular, our application spawns $p$ processes via the usual \texttt{mpirun} utility, which can land on up to $p$ SMP nodes. The number of processes per node depends on the specific specs of the host machines and on details of the experiment. A few underlying libraries used by our application (e.g., libtorch and mkldnn) spawn up to $N_t$ local threads of their own, where $N_t$ can be controlled via the OMP\_NUM\_THREADS environment variable. 

\begin{figure}[!ht]
  \centering
  \includegraphics[width=0.45\textwidth]{Figures/hybrid_distribution.png}
  \caption{Process-to-process hybrid distribution paradigm: processes communicate via MPI, and spawn local threads of their own that communicate via OpenMP inside an SMP node. MPI routines are only invoked outside of OpenMP parallel regions.  \label{fig:hybrid_distribution}}
\end{figure}

\subsection{Complexities}
\label{subsec:complexities}
In this sub-section, we will discuss computation and communication complexities of our approach. As shown in Figure \ref{fig:dl_parallel}, the entire data set with $N_s$ samples is split into $N_b$ mini-batches with $b_s$ samples per mini-batch. Each MPI task computes loss and gradients for the local mini-batch of size $b_s^{loc}$. Loss and gradient computations have a complexity of 
\begin{equation}
O\left(F(N_w,b_s^{loc}) + B(N_w, b_s^{loc})\right).
\end{equation}
Forward ($F$) and backward ($B$) propagation complexities are non-linear functions of $N_w$, $b_s^{loc}$, number of cores allocated per MPI task and the network architecture. We use libtorch C++ APIs to execute forward and backward propagation in a single MPI task, which internally uses MKLDNN \cite{mkldnn} for optimal performance on Intel CPUs. %Discussion of these non-linear functions is beyond the scope of this paper. 
Local gradients are averaged using  \emph{MPI\_Allreduce}, which has a communication complexity of $O(N_w + log(p))$. Since $N_w\gg  p$, we expect the communication time to remain almost constant, independent of $p$ and of the underlying algorithm used by the OpenMPI implementation. Network weights on each process are updated using this averaged gradient via a stochastic gradient descent (SGD) method. Synchronization of statistics for all batch normalization layers after each epoch has a complexity of  $O(N_w)$. The overall complexity per epoch is, therefore,
\begin{equation}
    O\left(N_b\left(F(N_w,b_s^{loc})+ B(N_w,b_s^{loc}) + N_w \right) \right).
\end{equation}

\subsection{Comparison to Open Source Software}
\label{subsec:comparison_to_oss}
\textit{\textbf{Tensorflow}} and \textit{\textbf{Pytorch}} are the most popular open source libraries for deep learning, and both provide support for distributed deep learning. Out of the box, they handle all-reduce operations on gradients computed on a local mini-batch on each device. \textit{\textbf{Horovod}} is an open source library \cite{sergeev_horovod} from Uber that enables data parallelism and gradient averaging. However, optimal load balancing, guarantees of loss independence on processor count, $p$ (Figure \ref{fig:loss_vs_epoch_256x256}), synchronized batch normalization and hybrid distributed implementation discussed in the previous sections are not provided out of the box by these open source libraries. Our framework democratizes the ability of data scientists to train models that are too big for GPUs with desired system performance and convergence rates without any distributed and high performance computing experience.

\begin{table}[!ht]
  \begin{center}
    \begin{tabular}{|c|c|c|c|c|} % <-- Alignments: 1st column left, 2nd middle and 3rd right, with vertical lines in between
      \hline
      %\textbf{Out of the box functionality} & \textbf{Tensorflow} & \textbf{Pytorch} &
      \shortstack{\textbf{Out of the box} \\ \textbf{functionality}} & \textbf{Tensorflow} & \textbf{Pytorch} &
       \textbf{Horovod} & \textbf{SciDDL}\\
      \hline
      %Gradient Average using All Reduce & Yes & Yes & Yes & Yes \\
      \shortstack{All reduce on \\Gradient} & Yes & Yes & Yes & Yes \\
      \hline
      %Load balancing & No & No & No & {\bf Yes} \\
      \shortstack{Loss Integrity \\ independent of $p$} & No & No & No & {\bf Yes} \\
      \hline
      %Synchronized Batch Normalization & No & No & No & {\bf Yes} \\
      \shortstack{Synchronized \\ Batch Normalization} & No & No & No & {\bf Yes} \\
      \hline
    \end{tabular}
    \caption{Qualitative comparison of SciDDL functionality with Open Source Software \label{tab:oss_comparison}}
  \end{center}
\end{table}


==> previous_work/algo_development_revised.tex <==

GPUs remain the overwhelmingly popular compute platform for training these models. GPU memory utilization during training is driven by three factors: 1) number of model parameters in the network, 2) mini-batch size, and 3) size of intermediate tensors created during loss and gradient computations. A known limitation of GPUs is their relatively small available memory: for example, a state-of-the-art NVIDIA Tesla V100 GPU has only 32GB memory. Peak memory utilization to train a DiffNet for domain size $512 \times 512$ and mini-batch size 64 is $\sim$64GB, which is twice the available GPU memory. Due to these memory limitations, training on GPUs is done using mini-batches as small as 16, which in turn results in slow convergence and prohibitive wall-clock times. On Table \ref{tab:gpu_runtimes_memory}, we show maximum batch size and GPU memory utilization for different domain sizes that we were able to train on a NVIDIA Tesla RTX with 24GB memory. \textit{DiffNet training on domain sizes $> 512 \times 512$ is not feasible on currently available GPUs including Tesla V100}.
 \begin{table}[!ht]
  \begin{center}
    \begin{tabular}{|c|c|c|c|}
    \hline
     {\bf Domain Size} &  {\bf Batch Size} & {\bf GPU Memory (GB)} & {\bf Time/Epoch (s)}\\
     \hline
     128$\times$128 & 16	& 0.7 & 105\\
     \hline
     256$\times$256	& 16	& 2.1 & 340\\
     \hline
     512$\times$512	& 16	& 16.4 & 1401\\
     \hline
\end{tabular}
\caption{GPU  memory utilization and time per epoch for 4096 samples for different domain and batch sizes. On Titan RTX with 24GB memory, Diffnet training on domain sizes $> 512 \times 512$ with batch size 16 is not feasible. \label{tab:gpu_runtimes_memory}}
\end{center}
\end{table}

NVIDIA AI Servers like DGX-2 can accommodate bigger batch sizes by distributing the batches across multiple GPUs in a single unit with more cumulative GPU memory (256GB with 8 GPUs and 32GB/GPU). However, they come with an expensive price tag of $\sim$\$0.5M and are not affordable for the general practitioner. In spite of this price tag, the maximum available memory \textbf{is still the same} as the cumulative memory available on 1 or 2 nodes of a CPU cluster.
 
In order to overcome those memory limitations, our \emph{SciDDL} framework is based on \emph{data parallel} distributed training on multi-node CPU clusters with 5-10x more memory-per-node than a single GPU, and multiple cores-per-node connected via high-end interconnects with low latency and high bandwidth, which can match or exceed the performance of single GPU. \textcolor{blue}{In addition to \textit{data parallelism}, extension to \textit{model parallelism} can further push the envelope on accessible network sizes. This is currently work in progress, and at the time of submission, we have insufficient results to report.}

The rest of this section is organized as follows: in section \ref{subsec:data_parallel_ddl} we provide details on data parallel training; in section \ref{subsec:sync_bn} we discuss the need for synchronized batch normalization; the OpenMP and MPI based hybrid distribution model is explained in section \ref{subsec:hybrid_distribution_model}; time complexities for computation and communication are discussed in section \ref{subsec:complexities}, and a comparison to open-source software is made in section \ref{subsec:comparison_to_oss}. In Table \ref{tab:notations}, we summarize the notations used in this section. 

\begin{table}[!ht]
  \begin{center}
    \begin{tabular}{|cc|}
    \hline
     $N_s$ & Total number of samples \\
     $b_s$ & Number of samples in a mini-batch \\
     $N_s^{loc}$ & Local number of samples \\
     $b_s^{loc}$ & Local mini-batch size \\
     $N_b$ & Number of mini-batches \\
     $N_w$ & Number of weights in the model \\
     $p$   & Number of MPI tasks in \emph{comm} \\
     $N_t$ & Number of threads per MPI task \\
     $F$   & Forward propagation complexity \\
     $B$   & Backward propagation complexity \\
     $L$   & Loss function \\
     $\theta$ & Model parameters \\
     $G_\theta$ & Gradient w.r.t model parameters \\
     \hline
\end{tabular}
\caption{Notations used in this section \label{tab:notations}}
\end{center}
\end{table}

\subsection{Data Parallel Distributed Deep Learning}
\label{subsec:data_parallel_ddl}
We use the {\it data parallel} strategy, where multiple replicas of a model are simultaneously trained to optimize a single objective function \cite{bennun_parallel_dnn}. In this approach, the training mini-batches are equally split among the available workers, as shown in Figure \ref{fig:dl_parallel}. Each of these workers asynchronously perform forward and back-propagation of their local mini-batch through the neural network. After each mini-batch, the locally computed gradients are averaged among workers via an {\it MPI\_Allreduce} operation, and that average is used by each local optimizer to update the layer parameters. The loss function is also computed locally, and the objective value is averaged among workers.
\begin{figure}[!ht]
  \centering
  \includegraphics[width=0.48\textwidth]{Figures/dl_dataparallel.png}
  \caption{Data Parallel Deep-Learning : multiple replicas of the model are asynchronously trained by workers, each worker using a subset of the global mini-batch. \label{fig:dl_parallel}}
\end{figure}

It is important that the samples (training examples) are split among workers in such a way that the same exact problem gets solved no matter the number of processes (MPI ranks). For that purpose, we adjust the total number of samples $N_s$ and the batch size $b_s$ to make them divisible by the number of workers $p$, such that the {\it local} sample count and batch size are given by
\begin{eqnarray}
N_s^{loc} = \ceil{\frac{N_s}{p}}, \\
b_s^{loc} = \floor{\frac{b_s}{p}}.
\end{eqnarray}
Furthermore, as shown in Figure \ref{fig:mini_batch_split}, each worker draws their local mini-batch sequentially from the global sample pool, in such a way that their union ({\it global} mini-batch) would equal the one used in a single-processor run with the same values of $N_s$ and $b_s$. This guarantees exactly identical results (modulo rounding errors due to gradient reduction) for any number of workers used. Finally, one can easily show that, when $N_s$ is not divisible by $b_s$, the remainder $N_s\mod b_s$ will still be divisible by $p$, which enforces optimal load balancing by guaranteeing that the local mini-batches processed by each worker at any given time have identical sizes.


\begin{figure}[!ht]
  \centering
  \includegraphics[width=0.48\textwidth]{Figures/mini_batch_split.png}
  \caption{Data splitting across workers in a parallel run: mini-batches are always guaranteed to have the same size across workers at any given time, promoting optimal load balance.\label{fig:mini_batch_split}}
\end{figure}

Algorithm \ref{alg:dl_parallel_algo} summarizes our per-epoch strategy for distributed training using the data parallel paradigm.
\begin{algorithm}[H]
%\KwResult{One epoch using data parallel training}
Generate $p N_s^{loc}$ samples, split in mini-batches of size $b_s^{loc}$\\
\For{$mb = 1$ \KwTo $N_b$} {
   {\bf x}_i \gets \{$b_s^{loc}$ samples\}                  \Comment{Worker $i$ local mini-batch}
   \ell_i(\theta) \gets L({\bf x}_i, G_\theta(\rvb, \nu))   \Comment{Forward pass and local loss}
   {\bf g}_i(\theta) \gets \nabla\ell_i(\theta)             \Comment{Back-prop and local gradient}
   \ell(\theta) \gets \frac{1}{p} \sum \ell_i(\theta)       \Comment{Average loss using MPI\_Allreduce}
   {\bf g}(\theta) \gets \frac{1}{p} \sum {\bf g}_i(\theta) \Comment{Average grad using MPI\_Allreduce}
   \Delta\theta \gets u({\bf g}, \theta, t)                 \Comment{Run local optimizer}\\
   \theta \gets \theta + \Delta\theta                       \Comment{Update network parameters}
}
\caption{Data parallel distributed deep learning (1 epoch)\label{alg:dl_parallel_algo}}
\end{algorithm}

\subsection{Synchronized Batch-normalization}
\label{subsec:sync_bn}
Batch Normalization (BN) is a procedure that dramatically improves the convergence of neural networks by re-scaling and re-centering data using running statistics, namely mean and variance, accumulated from each mini-batch in the course of an epoch \cite{ioffe_batchnorm}. This creates a dependency on the local mini-batch size, breaking the paradigm of problem independence on the number of workers discussed in section \ref{subsec:data_parallel_ddl}.
To remove this dependency, we developed a scheme to synchronize the mean and variance statistics at all BN layers by performing an {\it MPI\_Allreduce} operation after each epoch. This is especially important when the local mini-batch size on each processor is small, which would result in poor statistics and have a negative impact on validation accuracy. The BN synchronization scheme is explained in Algorithm \ref{alg:dl_bn_sync}.

\begin{algorithm}[H]
\ForEach{$\textrm{epoch}$} {
\ForEach{$\textrm{BN layer in network}$} {
\If{\textrm{in evaluation}} {
   \mu_{\mathcal{B}} \gets \frac{1}{p} \sum_i^p \mu_{\mathcal{B}}^{(i)} \Comment{Allreduce BN means}
   \sigma_{\mathcal{B}}^2 \gets \frac{1}{p} \sum_i^p {\sigma_{\mathcal{B}}^2}^{(i)} \Comment{Allreduce BN variances}
}}}
\caption{Batch-normalization synchronization algorithm\label{alg:dl_bn_sync}}
\end{algorithm}

\subsection{Hybrid Distribution Model}
\label{subsec:hybrid_distribution_model}
Our parallel distribution scheme is based on the so called {\it hybrid} MPI-OpenMP programming paradigm, in which communication between processes is done via MPI, while each process can spawn its own OpenMP threads that run inside a single shared-memory processor (SMP) node, as illustrated in Figure \ref{fig:hybrid_distribution}. Furthermore, since the OpenMP threads only communicate with other threads within the same SMP node, and MPI routines are only invoked outside of OpenMP parallel regions, our distribution scheme can be said to model the {\it process-to-process} hybrid paradigm.
In particular, our application spawns $p$ processes via the usual \texttt{mpirun} utility, which can land on up to $p$ SMP nodes. The number of processes per node depends on the specific specs of the host machines and on details of the experiment. A few underlying libraries used by our application (e.g., libtorch and mkldnn) spawn up to $N_t$ local threads of their own, where $N_t$ can be controlled via the OMP\_NUM\_THREADS environment variable. 

\begin{figure}[!ht]
  \centering
  \includegraphics[width=0.45\textwidth]{Figures/hybrid_distribution.png}
  \caption{Process-to-process hybrid distribution paradigm: processes communicate via MPI, and spawn local threads of their own that communicate via OpenMP inside an SMP node. MPI routines are only invoked outside of OpenMP parallel regions.  \label{fig:hybrid_distribution}}
\end{figure}

\subsection{Complexities}
\label{subsec:complexities}
In this sub-section, we will discuss computation and communication complexities of our approach. As shown in Figure \ref{fig:dl_parallel}, the entire data set with $N_s$ samples is split into $N_b$ mini-batches with $b_s$ samples per mini-batch. Each MPI task computes loss and gradients for the local mini-batch of size $b_s^{loc}$. Loss and gradient computations have a complexity of 
\begin{equation}
O\left(F(N_w,b_s^{loc}) + B(N_w, b_s^{loc})\right).
\end{equation}
Forward ($F$) and backward ($B$) propagation complexities are non-linear functions of $N_w$, $b_s^{loc}$, number of cores allocated per MPI task and the network architecture. We use libtorch C++ APIs to execute forward and backward propagation in a single MPI task, which internally uses MKLDNN \cite{mkldnn} for optimal performance on Intel CPUs. %Discussion of these non-linear functions is beyond the scope of this paper. 
Local gradients are averaged using  \emph{MPI\_Allreduce}, which has a communication complexity of $O(N_w + log(p))$. Since $N_w\gg  p$, we expect the communication time to remain almost constant, independent of $p$ and of the underlying algorithm used by the OpenMPI implementation. Network weights on each process are updated using this averaged gradient via a stochastic gradient descent (SGD) method. Synchronization of statistics for all batch normalization layers after each epoch has a complexity of  $O(N_w)$. The overall complexity per epoch is, therefore,
\begin{equation}
    O\left(N_b\left(F(N_w,b_s^{loc})+ B(N_w,b_s^{loc}) + N_w \right) \right).
\end{equation}

\subsection{Comparison to Open Source Software}
\label{subsec:comparison_to_oss}
\textit{\textbf{Tensorflow}} and \textit{\textbf{Pytorch}} are the most popular open source libraries for deep learning, and both provide support for distributed deep learning. Out of the box, they handle all-reduce operations on gradients computed on a local mini-batch on each device. \textit{\textbf{Horovod}} is an open source library \cite{sergeev_horovod} from Uber that enables data parallelism and gradient averaging. However, optimal load balancing, guarantees of loss independence on processor count, $p$ (Figure \ref{fig:loss_vs_epoch_256x256}), synchronized batch normalization and hybrid distributed implementation discussed in the previous sections are not provided out of the box by these open source libraries. 

Our framework democratizes the ability of data scientists to train models that are too big for GPUs with desired system performance and convergence rates without any distributed and high performance computing experience.

\begin{table}[!ht]
  \begin{center}
    \begin{tabular}{|c|c|c|c|c|} % <-- Alignments: 1st column left, 2nd middle and 3rd right, with vertical lines in between
      \hline
      %\textbf{Out of the box functionality} & \textbf{Tensorflow} & \textbf{Pytorch} &
      \shortstack{\textbf{Out of the box} \\ \textbf{functionality}} & \textbf{Tensorflow} & \textbf{Pytorch} &
       \textbf{Horovod} & \textbf{SciDDL}\\
      \hline
      %Gradient Average using All Reduce & Yes & Yes & Yes & Yes \\
      \shortstack{All reduce on \\Gradient} & Yes & Yes & Yes & Yes \\
      \hline
      %Load balancing & No & No & No & {\bf Yes} \\
      \shortstack{Loss Integrity \\ independent of $p$} & No & No & No & {\bf Yes} \\
      \hline
      %Synchronized Batch Normalization & No & No & No & {\bf Yes} \\
      \shortstack{Synchronized \\ Batch Normalization} & No & No & No & {\bf Yes} \\
      \hline
    \end{tabular}
    \caption{Qualitative comparison of SciDDL functionality with Open Source Software \label{tab:oss_comparison}}
  \end{center}
\end{table}

\textcolor{blue}{We were made aware of a recently released package \textbf{LBANN} which has similar capabilities as \textbf{SciDDL}. LBANN has model as well as data parallelism with multi-GPU capability, while model parallelism is work-in-progress for us. An additional distinction is our focus on incorporating higher order optimization methods (L-BFGS) for large batch training (see Fig.~\ref{fig:loss-epoch-plots-128x128}(bottom) and appendix for some results), along with batch synchronization. Our long term vision for SciDDL is sufficiently distinct from LBANN to suggest continued development of SciDDL with a niche application foci on Scientific ML}   
%We were unaware of this (fantastic) effort. After a thorough evaluation of LBANN,  we have identified several complementary strengths of LBANN and our SciDDL framework. The key capabilities that SciDDL does not (currently) have, that LBANN has are (a) model parallelism, and (b) multi-GPU training. The key capability that SciDDL has, that LBANN does not (currently) have include higher order optimization methods (L-BFGS) for large batch training, along with batch synchronization. We are currently actively developing capability for model parallelism and multi-CPU-GPU training (and will look to combine some efforts with the LBANN folks). Our long term vision for SciDDL is  sufficiently distinct from LBANN to suggest continued development of SciDDL with a niche application foci on Scientific ML. 
